Bucket Renormalization for Approximate Inference

Probabilistic graphical models are a key tool in machine learning applications. Computing the partition function, i.e., normalizing constant, is a fundamental task of statistical inference but it is generally computationally intractable, leading to extensive study of approximation methods. Iterative variational methods are a popular and successful family of approaches. However, even state of the art variational methods can return poor results or fail to converge on difficult instances. In this paper, we instead consider computing the partition function via sequential summation over variables. We develop robust approximate algorithms by combining ideas from mini-bucket elimination with tensor network and renormalization group methods from statistical physics. The resulting "convergence-free" methods show good empirical performance on both synthetic and real-world benchmark models, even for difficult instances.

==> _GM Renormalization (new) (2)/alg1.tex <==
\begin{algorithm}[ht!]
\caption{Mini-bucket renormalization (MBR)}
\label{alg:mbr}
\begin{algorithmic}[1]
\STATE {\bf Input:} GM $\mathcal M^{\dagger} = (\mathcal{G}^{\dagger}, \mathcal{F}^{\dagger})$, 
%with graph $\mathcal{G}^{\dagger}=(\mathcal{V}^{\dagger}, \mathcal{E}^{\dagger})$,  
elimination order $o$ and induced width bound $ibound$.
\vspace{0.05in}
  \hrule
    \vspace{0.05in}
\STATE 
$\mathcal{F} \leftarrow \mathcal{F}^{\dagger}$
\FOR{$i$ in $o$}
\STATE $\mathcal{B}_{i} 
\leftarrow \{\eff_{\alpha}|\eff_{\alpha}\in \mathcal{F}, i \in \alpha \}$
\STATE Divide $\mathcal{B}_{i}$ into $m_{i}$ subgroups $\{\mathcal{B}_{i}^{\ell}\}_{\ell=1}^{m_{i}}$ such that 
$|\mathcal{V}(\mathcal{B}_{i}^{\ell})|\leq ibound +1$ for  $\ell=1,\cdots,m_{i}$. 
%\FOR{$\ell = 1,\cdots, m_{i}-1$}
\FOR{$\ell=1,\cdots,m_{i}-1$}
\STATE Generate compensating factors $r_{i}^{\ell}, r_{i^{\ell}}$ 
by \eqref{eq:mbropt}.
\STATE Generate new factor $\eff_{\mathcal{B}_{i}^{\ell}\setminus\{i\}}$ 
by \eqref{eq:mbr1}.
\ENDFOR
\STATE Generate new factor $\eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}$ by \eqref{eq:mbr2}.
\FOR{$\ell=1,\cdots, m_{i}$}
\STATE $\mathcal{F} \leftarrow \mathcal{F} \cup \{\eff_{\mathcal{B}_{i}^{\ell}\setminus\{i\}}\}\setminus \mathcal{B}_{i}^{\ell}$
\ENDFOR
\ENDFOR
\vspace{0.05in}
  \hrule
  \vspace{0.05in}
\STATE {\bf Output:} $Z=\prod_{\eff_{\alpha}\in \mathcal{F}}\eff_{\alpha}$
\end{algorithmic}
\end{algorithm}

\iffalse
:
\begin{equation*}
\eff_{\mathcal{B}_{i}^{\ell}\setminus\{i\}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}\setminus\{i\}})
= 
\sum_{x_{i^{\ell}}}
r_{i^{\ell}}(x_{i^{\ell}})\prod_{\eff_{\alpha}
\in \mathcal{B}_{i}^{\ell}}
\eff_{\alpha}(x_{i^{\ell}}, \mathbf{x}_{\alpha\setminus\{i\}}).
\end{equation*}
\fi

\iffalse
\begin{align*}
\min_{r_{i}^{\ell}, r_{i^{\ell}}} \qquad
\sum_{\mathbf{x}_{\mathcal{B}_{i}^{\ell}}}
\bigg(
\eff_{\mathcal{B}_{i}^{\ell}} 
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) 
-
\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}} 
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}})
\bigg)^{2},
\end{align*} 
where $\eff_{\mathcal{B}_{i}^{\ell}} = \prod_{\eff_{\alpha}\in\mathcal{B}_{i}^{\ell}}\eff_{\alpha}$ and \begin{equation*}
\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) = 
    r_{i}^{\ell}(x_{i})
\sum_{x_{i^{\ell}}}
r_{i^{\ell}}(x_{i^{\ell}})
\eff_{\mathcal{B}_{i}^{\ell}}(x_{i^{\ell}}, \mathbf{x}
_{\mathcal{B}_{i}^{\ell}\setminus\{i\}}).
\end{equation*}
\fi
%\ENDFOR

==> _GM Renormalization (new) (2)/alg2.tex <==
\begin{algorithm}[ht!]
\caption{GM renormalization}
\label{alg:mbr_renormalization}
\begin{algorithmic}[1]
\STATE {\bf Input:} GM $\mathcal M^{\dagger} = (\mathcal{G}^{\dagger}, \mathcal{F}^{\dagger})$, 
%with graph $\mathcal{G}^{\dagger}=(\mathcal{V}^{\dagger}, \mathcal{E}^{\dagger})$, 
elimination order $o$ and induced width bound $ibound$.
\vspace{0.05in}
  \hrule
    \vspace{0.05in}
\STATE $\mathcal{M}^{(1)}\leftarrow \mathcal{M}^{\dagger}$
\STATE Run Algorithm \ref{alg:mbr} with 
input $\mathcal M^{(1)}, o, ibound$ to obtain mini-buckets  $\mathcal{B}_{i}^{\ell}$ and compensating factors $r_{i}^{\ell}, r_{i^{\ell}}$ for $i=1,\cdots, n$ and $\ell = 1,\cdots,m_{i}$.
\FOR{$\eff\in\mathcal{F}^{(1)}$}
\STATE Assign scope $\mathcal{S}_{\eff}$ for $\eff$ by \eqref{eq:initscope}. 
\ENDFOR
\FOR{$i$ in $o$}
\FOR{$\ell = 1,\cdots, m_{i}-1$}
\FOR{$\eff \in \mathcal{B}_{i}^{\ell}$}
\STATE Renormalize scope $\mathcal{S}_{\eff}$ for $\eff$ into $\widetilde{\mathcal{S}}_{\eff}$ by \eqref{eq:factorrenorm}.
\ENDFOR
\STATE Set $t = \sum_{j=1}^{i-1}(m_{i}-1) + \ell$. 
\STATE Renormalize GM $\mathcal{M}^{(t)}$ into $\mathcal{M}^{(t+1)}$ by \eqref{eq:gmrenorm}.
\STATE Assign scope 
$\mathcal{S}_{\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}}$ for factor $\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}$ 
by \eqref{eq:factorscope1}.
\ENDFOR
\STATE Assign scope 
$\mathcal{S}_{\eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}}$ 
for factor $\eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}$ 
by \eqref{eq:factorscope2}.
\ENDFOR
\vspace{0.05in}
  \hrule
  \vspace{0.05in}
\STATE {\bf Output:} Final GM $\mathcal M^{(T+1)}$ with $T = \sum_{i=1}^{n}(m_{i}-1)$.
\end{algorithmic}
\end{algorithm}
\iffalse
as follows
\begin{align*}
\mathcal{V} &\leftarrow \mathcal{V}\cup \{i^{\ell}\},\\
\mathcal{E} &\leftarrow \mathcal{E}
\setminus\mathcal{E}_{\mathcal{B}_{i}^{\ell}}
\cup \widetilde{\mathcal{E}}_{\mathcal{B}_{i}^{\ell}}
\cup \{\{i\}, \{i^{\ell}\}\} 
,\\
\mathcal{F} &\leftarrow \mathcal{F} 
\setminus\mathcal{F}_{\mathcal{B}_{i}^{\ell}}
\cup \widetilde{\mathcal{F}}_{\mathcal{B}_{i}^{\ell}}
\cup \{r_{i}^{\ell}, r_{i^{\ell}}\}, 
\end{align*}
\fi
\iffalse
as follows:
\begin{align*}
\mathcal{G}_{\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}}
&\leftarrow
(
\widetilde{\mathcal{V}}_{\mathcal{B}_{i}^{\ell}}
\setminus \{i\} ,
\widetilde{\mathcal{E}}_{\mathcal{B}_{i}^{\ell}}
\cup \{\{i^{\ell}\}\}
),\\
\mathcal{F}_{\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}} 
&\leftarrow
\widetilde{\mathcal{F}}_{\mathcal{B}_{i}^{\ell}}
\cup \{r_{i^{\ell}}\}.
\end{align*}
\ENDFOR
as follows:
\begin{align*}
\mathcal{G}_{\eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}}
&\leftarrow 
(
\mathcal{V}_{\mathcal{B}_{i}^{m_{i}}}, 
\mathcal{E}_{\mathcal{B}_{i}^{m_{i}}}
\cup \{\{i\}\}
), \\
\mathcal{F}_{\eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}} 
&\leftarrow
\mathcal{F}_{\mathcal{B}_{i}^{m_{i}}}
\cup \{r_{i}^{\ell}\}_{\ell=1}^{m_{i}-1}
. 
\end{align*} 
\fi

\iffalse
\STATE Assign scope for mini-bucket $\mathcal{B}_{i}^{\ell}$ as follows:
\begin{equation*}
    M_{i}^{\ell}
    \leftarrow 
    (
    (
    \bigcup_{\eff\in\mathcal{B}_{i}^{\ell}}
    \mathcal{V}_{\eff}
    ,
    \bigcup_{\eff\in\mathcal{B}_{i}^{\ell}}
    \mathcal{E}_{\eff}
    ),
    \bigcup_{\eff\in\mathcal{B}_{i}^{\ell}}
    \mathcal{F}_{\eff}
    )
\end{equation*}
\STATE Renormalize $M_{i}^{\ell}$ as follows:
\begin{align*}
    \widetilde{M}_{i}^{\ell}
    &\leftarrow
    (
    \widetilde{\mathcal{G}}_{i}^{\ell},
    \widehat{\mathcal{F}}_{i}^{\ell} 
    \cup \{r_{i^{\ell}}, r_{i^{\ell}}\}
    ),\\
    \widetilde{\mathcal{G}}_{i}^{\ell} 
    &\leftarrow 
    (
    \mathcal{V}_{\mathcal{B}_{i}^{\ell}} \cup \{i^{\ell}\}, 
    \widehat{\mathcal{E}}_{i}^{\ell}
    \cup \{\{i^{\ell}\}, \{i\}\}
    ).
\end{align*} 
\fi

==> _GM Renormalization (new) (2)/alg3.tex <==
\begin{algorithm}[ht!]
\caption{Global-Bucket Renormalization (GBR)}
\label{alg:lbr}
\begin{algorithmic}[1]
\STATE {\bf Input:} GM $\mathcal{M}^{\dagger} = (G^{\dagger}, \mathcal{F}^{\dagger})$, 
%with graph $G^{\dagger}=(\mathcal{V}^{\dagger}, \mathcal{E}^{\dagger})$, 
elimination order $o$ and induced width bound $ibound$.
\vspace{0.05in}
  \hrule
    \vspace{0.05in}
\STATE Run Algorithm \ref{alg:mbr_renormalization} 
with input $\mathcal{M}^{\dagger}, o, ibound$ to 
obtain renormalized GM $\mathcal{M}$ 
and compensating factors $r_{i}^{\ell}$ 
for $i=1,\cdots, n$ and $\ell = 1,\cdots,m_{i}$.
\STATE Set the renormalized elimination order as follows:
\begin{equation*}
\widetilde{o} = 
[1^{1},\cdots,1^{m_{1}-1}, 1, \cdots, n^{1},\cdots, n^{m_{n}-1}, n].
%\widetilde{o} = 1^{1},\cdots,1^{m_{1}},\cdots,n^{1},\cdots, n^{m_{n}}.
\end{equation*}
\FOR{$i^{\ell}= n^{m_{n}-1},\cdots,n^{1},\cdots, 1^{m_{1}-1},\cdots,1^{1}$}
\STATE Generate $s_{i}^{\ell}, s_{i}^{\ell}$ by solving 
\begin{align*}
    \min_{s_{i}^{\ell}, s_{i^{\ell}}}& \sum_{x_{i}^{(1)},x_{i}^{(2)}}
    \bigg(
    g_{i}(x_{i}^{(1)}, x_{i}^{(2)}) 
    -
    \widetilde{g}_{i}(x_{i}^{(1)}, x_{i}^{(2)}) 
    \bigg)^{2},
\end{align*}
\STATE where $g_{i}, \widetilde{g}_{i}$ is defined as follows:
\begin{align*}
g_{i}(x_{i^{\ell}}, x_{i}) 
&= 
\sum_{\mathbf{x}_{\mathcal{V}\setminus \{i,i^{\ell}\}}}
\prod_{\eff_{\alpha} \in \mathcal{F}\setminus \{r_{i}^{\ell}, r_{i^{\ell}}\}}\eff_{\alpha}(\mathbf{x}_{\alpha}), \\
\widetilde{g}_{i}(x_{i^{\ell}}, x_{i}) 
    &=  
    s_{i}^{\ell}(x_{i^{\ell}})
    \sum_{x_{i}^{\ell}}
    s_{i^{\ell}}(x_{i}^{\ell})
    g_{i}(x_{i}^{\ell}, x_{i}), 
\end{align*}
with its computation done by BE with elimination order of 
$\widetilde{o}\setminus \{i, i^{\ell}\}$.
\STATE Update GM $\mathcal{M}$ by $\mathcal{F}\leftarrow\mathcal{F}\setminus \{r_{i}^{\ell}, r_{i^{\ell}}\} \cup \{s_{i}^{\ell}, 
s_{i^{\ell}}\}$.
\ENDFOR
\STATE Get $Z = \sum_{\mathbf{x}}\prod_{\eff_{\alpha}\in \mathcal{F}}\eff_{\alpha}(\mathbf{x}_{\alpha})$ 
via BE with elimination order $\widetilde{o}$.
\vspace{0.05in}
  \hrule
  \vspace{0.05in}
\STATE {\bf Output:} $Z$
\end{algorithmic}
\end{algorithm}
\vspace{-0.1in}


==> _GM Renormalization (new) (2)/experiment.tex <==
%\vspace{-0.05in}
\section{Experimental Results}
\label{sec:experiment}
\begin{figure*}[ht!]
\vspace{-0.05in}
\begin{subfigure}[b]{0.245\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/ising_complete_delta.png}
    \vspace{-0.20in}
    \caption{Complete graph, $|\mathcal{V}|=15$}
    \label{fig:ising_complete_delta}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/ising_grid_delta.png}
    \vspace{-0.20in}
    \caption{Grid graph $15 \times 15$}% non-toroidal}%, $|\mathcal{V}|=225$}
    \label{fig:ising_grid_delta}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/ising_complete_ibound.png}
    \vspace{-0.20in}
    \caption{Complete graph, $|\mathcal{V}|=15$}
    \label{fig:ising_complete_ibound}
    \end{subfigure}
    \begin{subfigure}[b]{0.245\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/ising_grid_ibound.png}
    \vspace{-0.20in}
    \caption{Grid graph $15 \times 15$}%, $|\mathcal{V}|=225$}
    \label{fig:ising_grid_ibound}
    \end{subfigure}
    \vspace{0.1in}\\
    \begin{subfigure}[b]{0.249\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/ising_grid_time.png}
    \vspace{-0.20in}
    \caption{Grid graph $15 \times 15$}%, $|\mathcal{V}|=225$}
    \label{fig:ising_grid_time}
    \end{subfigure}
    \begin{subfigure}[b]{0.371\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/promedus.png}
    \vspace{-0.20in}
    \caption{Promedus dataset}
    \label{fig:promedus}
    \end{subfigure}
    \begin{subfigure}[b]{0.371\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/linkage.png}
    \vspace{-0.20in}
    \caption{Linkage dataset}
    \label{fig:linkage}
    \end{subfigure}
    \vspace{-0.3in}
    \caption{
    %\textcolor{red}{
    %\textbf{\subref{fig:ising_complete_delta}-\subref{fig:ising_grid_ibound}.} 
    Performance comparisons under (\subref{fig:ising_complete_delta}, \subref{fig:ising_grid_delta})
    varying interaction strength parameter $\Delta$, and (\subref{fig:ising_complete_ibound}, \subref{fig:ising_grid_ibound}) induced width bound $ibound$. 
    Ising models are either defined on  (\subref{fig:ising_complete_delta}, \subref{fig:ising_complete_ibound})  complete graphs
    with $|\mathcal{V}| = 15$ or (\subref{fig:ising_grid_delta}, 
    \subref{fig:ising_grid_ibound}) grid graphs 
    with $|\mathcal{V}| = 225$. 
    Each plot is averaged over $100$ models.
    (\subref{fig:ising_grid_time}) reports
    the averaged error versus elapsed time while varying $ibound$ in the same setting as (\subref{fig:ising_grid_ibound}),  
    where number labels by points % on each plot 
    indicate the corresponding $ibound$ used.
    %\textbf{\subref{fig:linkage}, \subref{fig:promedus}.}
    Numbers in brackets, e.g., MBR(19), 
    count the instances of each algorithm to win in 
    terms of approximation accuracy under
    %performance comparisons in 
    (\subref{fig:promedus}) Promedus  and  (\subref{fig:linkage}) Linkage  datasets. 
%    from UAI 2014 inference competition. 
    }
    %}
    \vspace{-0.1in}
\end{figure*}

In this section, we report experimental results on 
performance of our algorithms for approximating the partition function $Z$.
Experiments were conducted for 
Ising models defined on 
grid-structured and complete graphs
as well as two real-world datasets from the 
UAI 2014 Inference 
Competition \cite{uai}. 
We compare our 
mini-bucket renormalization (MBR) 
and global-bucket renormalization (GBR) scheme 
with 
other mini-bucket algorithms, 
i.e., mini-bucket elimination (MBE) by \citet{dechter2003mini} and 
weighted mini-bucket elimination (WMBE) by \citet{liu2011bounding}.
%, both providing upper bound for $Z$. 
Here, WMBE used uniform H\"older weights, 
with additional fixed point reparameterization updates 
for improving its approximation, 
as proposed by  
\citealp{liu2011bounding}. 
For all mini-bucket 
algorithms, 
we unified the choice of 
elimination order for 
each instance of GM 
by applying min-fill heuristics \cite{koller2009probabilistic}.
%\footnote{Min-fill repeatedly eliminates variables that result in the lowest 
%number of mini-buckets
%\cite{koller2009probabilistic}.}.
Further, 
we also run the 
popular variational inference algorithms: 
%for approximating $Z$: 
mean-field (MF) and loopy 
belief propagation (BP), 
\footnote{{MF and BP were implemented to 
run for $1000$ iterations at maximum. BP additionally used damping with $0.1$ ratio.}
}
For performance measure, 
we use 
the log-partition function error, 
i.e., 
$|\log_{10}Z - \log_{10}Z_{\text{approx}}|$ 
where $Z_{\text{approx}}$ 
is the approximated 
partition function 
from a respective algorithm.
%\textcolor{red}{
%We remark that the choice 
%of measure was 
%made to follow 
%\citealp{xue2016variable}, 
%for making easier 
%comparison with the 
%reported performance in 
%identical experiment setting.
%}
%add reason for $\log 10$


{\bf Ising models.}
\iffalse
\begin{figure}
    \centering
    
    \vspace{0.1in}\\
    \begin{subfigure}[b]{0.99\linewidth}
    \centering
    \includegraphics[width=0.49\textwidth]{fig/ising_complete_ibound.png}
    \includegraphics[width=0.49\textwidth]{fig/ising_grid_ibound.png}
    \vspace{-0.05in}
    \caption{Varying induced width bound $ibound$.}
    \label{fig:ising_ibound}
    \end{subfigure}
    \caption{Performance comparisons under various parameters. 
    Ising models are defined on complete graphs with $|\mathcal{V}| = 15$ (left) and grid graphs with $|\mathcal{V}| = 225$ (right). Each plot is averaged over $100$ models.}
    \label{fig:ising}
\end{figure}
\fi
We first consider the most popular binary pairwise GMs, called Ising models \cite{onsager1944crystal}:
%are defined with 
%mixed interactions (spin glasses):
%\begin{equation*} 
    $p(\mathbf{x}) = \frac{1}{Z}\exp\left(\sum_{i\in \mathcal{V}}\phi_{i}x_{i} 
    + \sum_{(i,j)\in \mathcal{E}}\phi_{ij}x_{i}x_{j}\right),$
%\end{equation*} 
where $x_{i}\in \{-1, 1\}$. 
In our experiments, we draw 
$\phi_{ij}$ and $\phi_{i}$ 
uniformly from intervals of 
$[-\Delta, \Delta]$ and $[-0.1, 0.1]$ respectively,
where $\Delta$ is 
a parameter controlling the `interaction strength' 
%parameter that controls the 
%degree of interactions 
between variables. 
As $\Delta$ grows, 
the inference task 
is typically harder. 
Experiments were 
conducted in two settings: 
complete graphs with $15$ 
variables ($105$ pairwise factors), 
and $15 \times 15$ non-toroidal grid graphs ($225$ variables, $420$ pairwise factors). 
Both %of complete and grid 
%GMs 
settings have moderate tree-width, 
enabling exact computation of 
 the partition function 
%can be computed exactly in reasonable (though still large)
%time 
using BE
with induced widths of 15 and 16, respectively.
We 
%Experiments were conducted 
%with 
vary the interaction 
strength $\Delta$ and the  
induced width bound $ibound$ 
(for mini-bucket algorithms), 
where 
%with other parameter fixed by 
$ibound = 10$ and $\Delta=1.0$ are the default choices.
%respectively.
For each choice of parameters, results are obtained by averaging over 
100 random model instances. % under % with 
%the specified parameters. 

As shown in Figure \ref{fig:ising_complete_delta}%\ref{fig:ising_grid_delta} \ref{fig:ising_complete_ibound},
%and 
-\subref{fig:ising_grid_ibound}, 
both MBR and GBR %clearly 
perform impressively compared to MF and BP. %outperform other 
%algorithms 
%significantly. 
Notably, the relative outperformance %benefit 
of our methods compared to the earlier approaches 
increases with % as the 
%size of interaction 
%strength parameter 
$\Delta$ (more difficult instances),
and as the bound of induced width gets smaller. 
This suggests that 
our methods %the proposed algorithm 
scale well 
with the size and difficulty of GM. 
In Figure \ref{fig:ising_complete_ibound}, 
where $ibound$ is varied for complete graphs, 
we observe that GBR does not improve over MBR when 
 $ibound$ 
is small, 
but does so after 
$ibound$ grows large. 
This is consistent with our 
expectation that in order for 
GBR to improve over MBR, the 
initial quality of MBR 
should be acceptable.
%required to be 
%not too bad. 
Our 
experimental setup on Ising grid GMs with 
varying interaction strength is 
identical to that of %the experiment done in 
\citet{xue2016variable}, where they 
approximate variable 
elimination in the Fourier domain. 
Comparing results, 
one can observe that our methods
significantly outperform their prior algorithm.

Figure \ref{fig:ising_grid_time} 
reports the trade-off between 
accuracy and elapsed time with 
varying $ibound$. 
Here, we observe that 
MBR is much faster than MBE or WMBE to reach a 
desired accuracy, 
i.e., MBR with $ibound = 4$ 
is faster and more accurate than 
MBE and WMBE 
with $ibound > 4$. 
%Further, we also note that %In our experiments,
%in terms of complexity, 
%MBR with larger
%$ibound$ is more effective for running time 
%than running GBR for its improvement.
%in MBR 
%is observed to be 
%more efficient in our experiments
%than additionally 
%running GBR for improvement 
%since it typically requires 
%less time to run.
%However, 
%the memory usage in MBR always increase exponentially
%with respect to $ibound$, while
%GBR uses the same-order of memory with MBR of same $ibound$.
{
Further, 
we also note that 
increasing $ibound$ for GBR 
does not lead to 
slower running time, 
while the accuracy is improved. 
This is because smaller $ibound$ increases
the numbers of mini-buckets
and corresponding SVD calls. 
}


\iffalse
Our recommended 
strategy based on the results for 
applying mini-bucket 
schemes on 
larger-scale instances 
would be to increase the size of $ibound$ 
as large as possible (given memory resources), 
and then run GBR for 
additional improvement of accuracy,
without any 
further increase in order of 
memory size.
Finally, we remark that 
increasing $ibound$ 
may not necessarily lead to slower running time 
for MBR, GBR and WMBE, e.g., 
increasing from $ibound=2$ to $4$, 
while the accuracy is increased. 
This is because smaller $ibound$, i.e., 
larger number of mini-buckets, 
leads to more SVD calls to solve 
in MBR/GBR as well as more parameters 
to optimize in WMBE.
\fi
%, 
%and number of optimizations 
%to solve in GBR.
\iffalse
Here, we observe that MBE is 
the fastest, 
which is as expected since MBE 
is the most simple 
algorithm with worst performance. 
In next place, one can observe 
MBR to be in par with WMBE with superior 
approximation quality. 
This is because 
while MBR needs 
additional complexity 
for performing SVD on 
each mini-buckets, 
while WMBE requires 
additional 
message-passing schemes 
for finding fixed 
reparameterization points. 
Finally, GBR is the slowest 
with the best 
performance available for the same $ibound$. 
\fi


\iffalse
\subsection{UAI instances}
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.99\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/promedus.png}
    \vspace{-0.05in}
    \caption{promedus dataset}
    \label{fig:promedus}
    \end{subfigure}
    \vspace{0.1in}\\
    \begin{subfigure}[b]{0.99\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/linkage.png}
    \vspace{-0.05in}
    \caption{linkage dataset}
    \end{subfigure}
    \caption{Performance comparisons for various instances in promedus (top) and linkage (bottom) datasets from the 
    UAI 2014 inference competition. Numbers in bracket 
    indicate count of instances where each algorithm dominate in 
    terms of performance.}
    \label{fig:uai}
\end{figure}
\fi

{\bf UAI datasets.}
We further show results of 
real-world models 
from the UAI 2014 
Inference Competition, 
namely the Promedus (medical diagnosis)  
and Linkage (genetic linkage) 
datasets. 
Specifically, 
there exist $35$ instances of Promedus GMs in 
with the average of $544.75$ binary variables 
and $305.85$ non-singleton 
hyper-edges with 
averaged maximum size
$\max_{\alpha\in\mathcal{E}}|\alpha|=3$. 
In case of Linkage GMs, there exist 
$17$ instances with the average of $949.94$ variables 
with averaged maximum cardinality  $\max_{i\in\mathcal{V}}|\mathcal{X}_{i}| = 4.95$ 
and $727.35$ non-singleton 
hyper-edges with averaged maximum 
size $\max_{\alpha\in\mathcal{E}}|\alpha|=4.47$. 
Again, induced width bounds for mini-bucket algorithms are 
set to $ibound = 10$. 

The experimental results are 
summarized in Figure \ref{fig:promedus} 
and \ref{fig:linkage}. 
Here, results for MF was omitted since 
it is not able to 
run on these instances by its construction. 
First, in Promedus dataset, 
i.e., Figure \ref{fig:promedus}, 
MBR and GBR clearly 
dominates over all other algorithms. 
Even when GBR fails to improve 
MBR, it still outperforms other algorithms. 
Next, in Figure \ref{fig:linkage}, 
one can observe that MBR and GBR 
outperform other algorithms 
in $11/17= 64\%$ of 
the Linkage instances 
%\textcolor{red}{
and are always as nearly good as the best, i.e., BP, in other instances. %}
In particular, our algorithms 
outperform over all 
previous mini-bucket variants 
%at the cost of 
%loosing bounding property, 
and expected to outperform BP more significantly
by choosing a larger $ibound$. 
%Consequently, we conclude 
%that our algorithms outperform 
%even in real-world datasets and 
%they are universal, 
%i.e., works well in 
%various kinds of GMs.

\textbf{Guide for implementation.} 
Based on the experiments, 
we provide 
useful recommendations 
for application of MBR and GBR.
First, we emphasize that 
choosing the right elimination order 
is important for performance. 
Especially, min-fill heuristic 
improved the performance 
of MBR and GBR significantly, 
as with other mini-bucket algorithms. 
Further, whenever 
memory is available, 
running MBR with increased $ibound$ 
typically leads to better 
trade-off between complexity 
and performance 
than running GBR. 
When memory 
is limited, 
GBR is recommended for improving the approximation quality while using the same-order of memory. 


\iffalse
recommended 
strategy based on the results for 
applying mini-bucket 
schemes on 
larger-scale instances 
would be to increase the size of $ibound$ 
as large as possible (given memory resources), 
and then run GBR for 
additional improvement of accuracy,
without any 
further increase in order of 
memory size.
\fi


\iffalse
In this section,
we compare the proposed
truncating mini-bucket elimination (coined TMBE) to
other variants of bucket elimination, i.e.,
mini-bucket elimination for lower and upper bounding partition function (coined MBE-LB and  MBE-UB respectively)
and (unoptimized) weighted-mini-bucket elimination for 
lower and upper bounding partition function
(coined WMBE-LB and WMBE-UB respectively) and also the popular variational inference algorithms, mean-field (MF) and belief propagation (BP) algorithm.
We point out that TMBE, MBE, WMBE algorithms were not 
optimized with respect to any global properties of the
GM and thus much faster compared to the variationl algorithms, i.e., MF and BP.
For performance measure, we use the log-partition function error, i.e.,
$|\log \left(Z/Z_{\text{approx}}\right)|$ where $Z_\text{approx}$ is the
approximated partition function from the algorithms. 

\subsection{Experimental Setting}
\paragraph{Forney-style random factor models. }
Forney-style random factor models are 
generated as follows: 
the log-factors are drawn from the 
normal distribution, i.e., $\log \mathbf{F}_{\alpha}(\mathbf{x}_{\alpha})\propto \mathcal{N}(0,\Delta)$,
for all $\mathbf{x}_{\alpha}$.
Here, $\Delta \geq 0$ is the `variance parameter'
that controls variance of the random factors..
When $\Delta = 0$, variables are independent. 
As $\Delta$ grows,
the inference task is typically harder.
In this case, we assume 
a special structure on graphs whose
vertices and edges are represented by factors and
variables of the original GMs.
We remark that this does not correspond to the original
hypergraph defined with respect to the GM and 
does not permit any hyperedges.
Specifically, we consider grid and complete graphs. 

\paragraph{Random Ising models. } 
The next set of GMs we consider are random 
Ising models with nonzero magnetic fields.
To this end, Ising models were defined 
with mixed interactions (spin glasses):
\begin{equation*}
    p(\mathbf{x}) = \frac{1}{Z}\exp\left(\sum_{u\in\mathcal{V}} \phi_{u} x_{u} + \sum_{\{u,v\}\in E}\phi_{uv}x_{u}x_{i}\right),
\end{equation*}
where $x_{u}\in \{-1, 1\}$ and
$\phi_{uv}\sim \mathcal{N}(0,\Delta)$.
In this case, we vary $\Delta$ as the variance of Ising interaction
of GMs to see its effect. Again, we consider complete and grid graphs.

\paragraph{UAI Linkage instance.}
Finally, we consider two GMs from linkage and Pedigree in UAI 2014 competition respectively.
 The GM from Pedigree have $385$ binary 
variables, 
with non-pairwise factors. 
The GM from linkage have $1077$ variables with at most $3$ states, 
with non-pairwise factors.

\subsection{Experimental results} 
In order to investigate the performance of the algorithms in various situations, we varied the parameters of GM while keeping others fixed.
\paragraph{Varying graph size.}
\paragraph{Varying number of states.}
\paragraph{Varying variance parameter.}
\paragraph{Varying {\it mbound}.}

\iffalse
In the first set of experiments,
we consider small GMs with Forney-style assumptions
in order to observe the performance of TMBE
with respect to various properties of the GM. 
To this end, we consider Forney-style GMs with log-factors drawn from the
normal distribution, i.e., $\log \mathbf{F}_{\alpha}[\mathbf{x}_{\alpha}]\propto \mathcal{N}(0,T)$,
for all $\mathbf{x}_{\alpha}$.
Here, $T \geq 0$ is the `interaction strength' parameter
that controls the degree of interactions between variables.
When $T = 0$, variables are independent. As $T$ grows,
the inference task is typically harder.
In this case, we assume a special structure on graphs whose
vertices and edges are represented by factors and
variables of the original GMs.
We remark that this does not correspond to the original
hypergraph defined with respect to the GM.
See Figure \ref{fig:graphs} for
an illustration of such Factor-graph GMs.

Specifically,
we first consider binary GMs
associated with complete graph, and
varied its temperature and size
of the complete graph to observe its effect.
Temperature was varied with graph fixed as a
complete graph with size $4$, as shown in
Figure \ref{fig:graphs}.
The size of graph was varied by changing number of
factors in the complete graph and
temperature of the GM was fixed to $T=1.0$.
Next, we considered GMs
associated with $3\times 3$ grid graph,
and varied its temperature and number of states in
variables to observe its effect.
Again, temperature was varied with number of variable states
fixed to $2$, i.e., we considered binary variables.
Number of variable states were varied with
temperature of GM fixed to $T=1.0$.
See Figure \ref{fig:exp1} and \ref{fig:exp2} for the results. 
Here, one can observe TMBE outperforming all algorithms 
at the cost of loosing the bounding property.

Next, we consider large (symmetric) Ising model on $10\times10$ grid graph
to observe the performance of TMBE in large-scale instances.
To this end, Ising models were defined with mixed interactions (spin glasses):
\begin{equation*}
    p(\mathbf{x}) = \frac{1}{Z}\exp\left(\sum_{(u,v)\in E}\phi_{uv}x_{u}x_{i}\right),
\end{equation*}
where $x_{u}\in \{-1, 1\}$ and
$\phi_{uv}\sim \mathcal{N}(0,T)$.
In this case, we varied the temperature
of GMs to see its effect.
We remark that Ising model does not satisfy Forney-style assumption and
TMBE cannot be applied directly.
To overcome this, we applied TMBE after converting 
given Ising model into a equivalent Factor-graph GM satisfying the
Forney-style assumption by the 
procedure described in \eqref{eq:factor2forney}. 
Moreover, to enhance the performance of TMBE,
we introduced an additional heuristic to
avoid choosing the identity factor,
i.e., $\{\beta^{(i)}:i\in\mathcal{V}\}$ in \eqref{eq:factor2forney},
for performing truncated SVD
while truncating a variable.
The intuition is that truncated SVD is likely to perform worse
for an identity factor since its singular
values are equally significant.
See Figure \ref{fig:exp3} for the results. 
Here, one can see TMBE outperforming all algorithms, 
even though it was applied to a modified, Forney-style GM 
of size larger than the original GM.
\fi

\fi

==> _GM Renormalization (new) (2)/intro.tex <==
\section{Introduction}
Graphical Models (GMs) express the 
factorization of the joint multivariate 
probability distribution over subsets of variables 
via graphical relations among them. 
They have played an important role in many %machine learning applications or 
fields, including 
computer vision \cite{freeman2000learning}, 
speech recognition \cite{bilmes2004graphical},
social science \cite{scott2017social} and 
deep learning \cite{hinton2006reducing}.
%in a number of statistical disciplines including
%machine learning \cite{jordan1998learning,freeman2000learning},
%artificial intelligence \cite{pearl2014probabilistic},
%theoretical computer science \cite{bollobas1976cliques},
%information theory \cite{gallager1962low,kschischang1998iterative} and
%physics \cite{35Bet,36Pei,87MPZ,parisi1988statistical,09MM}.
Given a GM, computing the partition function $Z$ (the normalizing constant) is the essence of other statistical inference tasks such as marginalization and sampling. 
The partition function can be 
calculated efficiently in tree-structured GMs through an iterative (dynamic programming) algorithm eliminating, i.e. summing up, variables sequentially. In principle, the elimination strategy extends to arbitrary loopy graphs, but the computational complexity is exponential in the tree-width, e.g.,
the junction-tree method \cite{shafer1990probability}.
%however resulting in an exponentially difficult in their %graphical model 
%tree-width. %, of the corresponding junction-tree graph \cite{shafer1990probability}, thus intractable, computations. Moreover 
Formally, the computation task is 
\#P-hard even to approximate \cite{jerrum1993polynomial}.

Variational approaches are often the most popular practical choice for approximate computation of the partition function. 
They map the counting problem into an approximate optimization problem stated over
a polynomial (in the graph size) number of variables. The optimization is typically solved iteratively via a message-passing algorithm, e.g.,
%approximately. 
%Popular variational methods include: 
mean-field \cite{parisi1988statistical}, 
belief propagation \cite{pearl1982reverend}, 
tree-reweighted \cite{wainwright2005new}, 
 or %hybrids formulated in terms of optimization over the so-called
gauges and/or re-parametrizations \cite{ahn2017gauge, ahn2018gauged}.
Lack of accuracy control and difficulty in forcing convergence in an acceptable number of steps are, unfortunately, typical for hard GM instances. 
% Here, one of the key challenges is to scale them efficiently with respect to the number of optimization variables and the magnitude of model parameters. If they grow,
%for 
%variational methods 
%are to scale 
%efficiently with 
%the number of variables. 
%As this number grows, 
%optimization is hard and 
%message-passing algorithms  often suffer from  lack of convergence, and their performances should be inherently bad. 
%Utilizing 
Markov chain Monte Carlo methods (e.g., see  
\citealp{alpaydin2014introduction}) %or 
%search algorithms \cite{henrion1991search,viricel2016guaranteed, lou2017anytime} 
are also popular to approximate the partition function,
%It is preferable as asymptotically exact, 
but typically suffer, even more than variational methods,  from slow convergence/mixing.
%with the number of the generated samples (exponential in the system size for large, bad instances). 
% proned are alternative directions, but they tend to suffer even more in large models. Specifically, the former constructs a Markov chain to estimate the partition function from random samples, but its mixing is typically exponentially slow, and it provides an estimation with high variance. 
%The search algorithms are based on explicit enumeration of the conﬁgurations, which is, however, suited for only special type of problems, while even in these cases the quality of improvement is marginal 
%in the case of exponentially large search spaces. {\color{red} ... message not clear ... I would remove mentioning the search algorithms at all ...}

 
 
%Approximate elimination 
%algorithms have been studied. 
Approximate elimination is a sequential method to estimate the partition function.  Each step consists of summation over variables followed by (or combined with) approximation of the resulting complex factors. Notable flavors of this method include 
%Of the flavors , then followed by , consisting in 
%In another line of research, elimination algorithms aim to approximate the intractable sequential summations 
%over variables in GM of large tree-width for computing its partition function: 
%the process is approximated as either 
truncation of the Fourier coefficients \cite{xue2016variable}, approximation by random mixtures of rank-$1$ tensors \cite{wrigley2017tensor}, and arguably the most popular, 
elimination over mini-buckets \cite{dechter2003mini,liu2011bounding}. One advantage of the mini-bucket elimination approach is %related to, first of all, 
the ability to control the trade-off between computational complexity and approximation quality by
adjusting an induced-width parameter.  %that controls the size of mini-buckets, 
%i.e., if one chooses a larger parameter,  they run slower, but promise a better accuracy. 
Note that analogous control in variational methods, such as varying region sizes in generalized belief propagation  
\cite{yedidia2001generalized}, typically results in much more complicated optimization formulations to solve.
Another important advantage of mini-bucket elimination is that it is always guaranteed to terminate and, usually, it does so quickly. 
This is in contrast to iterative message-passing implementations of variational methods which can be notoriously slow on difficult instances. 
%typically much faster then related variational algorithms, simply because they are typically faster than iterative message-passing schemes as they are non-iterative and guarantee to terminate, i.e., have only a single round.  
%Finally, mini-bucket elimination provides a sensible (interpretable in terms of an effective/reduced GM) outcome even if stopped before the algorithm's completion. 
%robust: even if one terminates them before exploring all eliminations, 
%over mini-buckets, they still provide reasonable approximations to the partition function. 
%Other approximate 
%eliminations include 
%approximating the 
%variable elimination process 
%via 
%truncated Fourier 
%coefficients \cite{xue2016variable} 
%or mixtures of rank-$1$ tensors \cite{wrigley2017tensor}.

\iffalse
In another line of research, mini-bucket methods
\cite{dechter2003mini, liu2011bounding} 
aim to 
relax the intractable
sequential summations over 
variables in GM of large tree-width 
for computing its partition function:
they split the process into  
eliminations over ``mini-buckets''. 
The trade-off control between
their computational complexity and approximation quality
is easy using a small %clique size
induced-width 
parameter, i.e., if one chooses a larger parameter, 
they run slower, but promise a better accuracy.
Such a control in variational methods is harder as
they require to develop
new and more complex optimization tasks of 
a larger number of variables, 
e.g., region-based belief propagation 
\cite{yedidia2001generalized}.
More importantly, 
they are typically faster than 
iterative message-passing schemes as
they are non-iterative and 
guarantee to terminate, i.e., 
have only a single round.  
Even if one terminates them before 
exploring all eliminations over mini-buckets,
they still provide reasonable approximations to the partition function.
\fi
%; 
%results can be poor 
%with small cliques, 
%but larger cliques are 
%easily used to 
%improve its bounds. 
%Computational time for 
%the mini-buckets 
%scale well since 
%they are fast and non-iterative by 
%construction. 
%However they 
%may not perform 
%as well as variational 
%algorithms 
%since they tend to 
%make relatively 
%loose approximations on the 
%elimination process.

{\bf Contribution.} 
We improve the approximation quality of mini-bucket methods %by 
using tensor network and renormalization 
group approaches from statistical physics.
%In particular, 
%In another line of research, 
%we take advantage of the fact that the tensor networks allow a representation for the partition function.
%which is 
%different from the standard factor-graph representation. 
In this regard,  our method extends a series of recent papers 
exploring multi-linear tensor network transformations/contractions   
 %description for the partition function of a GM  via representing it as a collection of tensors connected by contractions, where several recent works 
\cite{novikov2014putting, wrigley2017tensor, ahn2017gauge, ahn2018gauged}.
%have employed this view and  utilized the corresponding multi-linear transformation. % to their benefit. 
More generally, tensor network renormalization 
algorithms \cite{levin2007tensor, evenbly2015tensor} 
have been proposed in the quantum and statistical physics literature
%renormalization 
%%group theory in physics 
for estimating partition functions. The algorithms consist of coarse-graining 
the graph/network by contracting sub-graphs/networks using a low-rank 
projection as a subroutine. 
However, %to date, 
the existing renormalization methods in the physics literature
have focused primarily on a %relatively 
restricted class of tensor-factorized models over regular grids/lattices,\footnote{
The special models are related to what may be called Forney-style grids/lattices \cite{forney2001codes} in the GM community.} while
factor-graph models \cite{clifford1990markov} over generic graphical structures
are needed in most machine learning applications. 


For generalizing them to factor-graph models,
one would face at two challenges:
%non-trivial mainly due to two reasons: 
(a) coarse-graining of the tensor network 
relies on the periodic structure of  
grid/lattices 
and (b) its low-rank projections are only 
defined on ``edge variables'' 
that allows only two adjacent factors. 
To overcome them, 
we first replace the coarse-graining step by 
sequential elimination 
of the mini-bucket algorithms,
%as a method 
%to contract the network, 
and then use the strategy of 
``variable splitting'' 
%semantics of the 
%mini-bucket algorithms 
in order to generate 
auxiliary edge variables. 
\iffalse
In this paper, we indeed propose
the tensor network renormalization 
framework, i.e., low-rank 
projections of factors, 
for general factor-graph models. 
Our main idea is on 
the mini-bucket approximation of 
variable elimination/graph contraction, which
can also be viewed as a generalization to what 
we call ``bucket renormalization''.
\fi
\iffalse
In this paper, we overcome the 
general graph limitation of the 
tensor network renormalization approaches. 
This improvement can also be viewed, 
from the mini-bucket perspectives, 
as a generalization to what 
we call ``bucket renormalization''.
\fi
\iffalse
While efficient, %their 
applications are 
limited since 
implementation of the 
algorithm relies on the  
special structure 
of the graph 
considered in physics.
Here, we introduce a new family of 
mini-bucket methods for GMs, 
transferring the essence of 
tensor network 
renormalization 
algorithms to 
GMs with general structures. 
Our algorithms 
interpret the procedure of 
tensor-network renormalization 
as a ``bucket renormalization'' 
with using low-rank 
approximation for the 
simplification process. 
\fi
Namely, we
combine ideas from tensor network renormalization and the mini-bucket schemes
where one is benefical to the other.
We propose two algorithms, which we call MBR and GBR: %, under the direction:
%the mini-bucket renormalization (MBR) and the global-bucket renormalization (GBR) schemes. 
\begin{itemize}
\item \emph{Mini-bucket renormalization} (MBR) consists of sequentially splitting summation over the current (remaining) set of variables into subsets --
multiple mini-buckets which are then  ``renormalized''. We show that this process is, in fact, equivalent to applying low-rank projections on the mini-buckets to approximate the variable-elimination process,  thus resulting in better approximation than the original mini-bucket methods. In particular, we show how to resolve approximate renormalization locally and efficiently through application of truncated singular value decomposition (SVD) over small matrices.

\item 
While MBR is based on a sequence of local low-rank approximations applied to the mini-buckets, 
 \emph{global-bucket renormalization} (GBR) extends MBR by approximating mini-buckets globally. %, 
%is motivated to design for improving MBR by incorporating global approximations on mini-buckets,
%Just like the previous mini-bucket schemes, 
%MBR is based on sequence 
%of local approximations. 
%Hence 
%this is expected to be 
%improved by 
%incorporating a global 
%perspective, 
%minimizing error in the partition function approximation more explicitly. 
This is achieved by first applying MBR to mini-buckets, then calibrating the choice of low rank projections by minimizing the partition function 
approximation error with respect to renormalization of the ``global-bucket''. 
Hence, GBR takes additional time to run but may be expected to yield better accuracy.

%Therefore, GBR should be considered as an improvement (over MBR) when the bare MBR is not perfect but still of satisfactory. 
\end{itemize}

%Even though we limit discussions of this manuscript to binary pair-wise GMs, 
Both algorithms are easily applicable to arbitrary GMs %including general GMs with 
with interactions (factors) of high orders, hyper-graphs and large alphabets.
We perform extensive experiments %on our newly developed algorithms 
on synthetic (Ising models on complete and grid graphs) and real-world models from the UAI dataset.
%These confirm our theoretical hypothesis: i
In our experiments, both MBR and GBR 
show performance 
%which is 
%universally 
superior to other state-of-the-art 
elimination and variational algorithms. 

==> _GM Renormalization (new) (2)/main_result.tex <==
\section{Mini-Bucket Renormalization}
\label{sec:rmbe}
We propose a new scheme, named 
mini-bucket renormalization
(MBR). Our approach 
approximates BE by 
splitting each 
bucket into 
several smaller 
mini-buckets to be 
``renormalized''. 
Inspired 
by tensor renormalization groups (TRG, \citealp{levin2007tensor}, see also references therein) in the physics literature, 
MBR utilizes low-rank approximations to
the mini-buckets instead of simply applying $\max$ (or $\min$) operations as in MBE. 
%Thus we lose guaranteed bounds on $Z$ but hope to gain accuracy. 
{Intuitively, MBR is similar to MBE 
but promises better accuracy.}
\iffalse
\textcolor{red}{This method can be seen as a 
generalization of TRGs in the 
physics literature \cite{levin2007tensor} 
to graphical models 
with arbitrary structure.}
\fi
%*Our method was inspired by work on TRGs in the physics literature (Refs)*

\iffalse
In this section,
%This section consists of two parts. 
we first provide the formal description 
of MBR.
Then, we provide an alternative 
interpretation of MBR as a sequence of 
GM renormalization scheme, 
resulting in an 
auxiliary GM 
with small induced width 
providing approximate inference 
via junction tree algorithm  \cite{kschischang1998iterative} . 
\fi
\begin{figure}[t!]
\vspace{-0.05in}
    \centering
    \begin{subfigure}[b]{0.99\linewidth}
    \centering
    \includegraphics[width=0.90\textwidth]{fig/mbr.png}
    \end{subfigure}
    \caption{Renormalization process for mini-buckets $\mathcal{B}_{1}^{a} = \{\eff_{12},\eff_{13}\},
    \mathcal{B}_{1}^{b} = \{\eff_{15},\eff_{16}\}$ and 
    $\mathcal{B}_{1}^{c} = \{\eff_{14}\}$.
    }
    \label{fig:mbr}
    \vspace{-0.1in}
\end{figure}
\subsection{Algorithm Description}
%Specifically, consider a
%GM $M = (G, \mathcal{F})$.
For each variable $i$ in the elimination order $o$, 
MBR partitions a 
bucket $\mathcal{B}_{i}$ into
$m_{i}$ distinct mini-buckets 
$\{\mathcal{B}_{i}^{\ell}\}_{\ell=1}^{m_{i}}$
with maximal size bounded by $ibound$. 
Then for $\ell = 1,\cdots, m_{i}-1$, 
mini-bucket $\mathcal{B}_{i}^{\ell}$ 
is ``renormalized'' through  
replacing vertex $i$ 
by its replicate $i^{\ell}$ 
and then introducing local factors $r_{i}^{\ell}, r_{i^{\ell}}$ for error compensation, i.e., 
\begin{equation*}
    \widetilde{\mathcal{B}}_{i}^{\ell} 
    \leftarrow 
    \{\eff_{\alpha \setminus \{i\} \cup \{i^{\ell}\}}| 
    \eff_{\alpha}\in\mathcal{B}_{i}^{\ell}\}
    \cup \{r_{i}^{\ell}, r_{i^{\ell}}\}.
\end{equation*}
%\textcolor{red}{
Here, $r_{i}^{\ell}, r_{i^{\ell}}$ 
are local 
``compensating/renormalizing 
factors'', 
chosen to approximate 
%the squared error of 
the factor  $\eff_{\mathcal{B}_{i}^{\ell}}=\prod_{\eff_{\alpha}\in\mathcal{B}_{i}^{\ell}}\eff_{\alpha}$
well, where MBE approximates it using \eqref{eq:mbemax} and \eqref{eq:mbesum}. 
{See Figure \ref{fig:mbr}
for illustration of the renormalization 
process.}
%, 
%induced from mini-bucket $\mathcal{B}_{i}^{\ell}$ on $\mathbf{x}_{\mathcal{B}_{i}^{\ell}}$. 
Specifically, the local compensating/renormalizing factors are chosen by 
solving the following optimization:
\begin{align}\label{eq:mbropt}
  \operatornamewithlimits{\mbox{min}}_{r_{i}^{\ell}, r_{i^{\ell}}}\qquad
    \sum_{\mathbf{x}_{\mathcal{B}^{\ell}_{i}}}
    \left(
    \eff_{\mathcal{B}_{i}^{\ell}}
    (\mathbf{x}_{\mathcal{B}_{i}^{\ell}})
    -
    \widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}
    (\mathbf{x}_{\mathcal{B}_{i}^{\ell}})
    \right)^{2},
\end{align}
where $\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}$ is the
factor induced on $\mathbf{x}_{\mathcal{B}_{i}^{\ell}}$ 
from the renormalized mini-bucket $\widetilde{\mathcal{B}}_{i}^{\ell}$: %, expressed as follows
\begin{align*}
    \widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}(\mathbf{x}_{\mathcal{B}_{i}^{\ell}})&= 
    \sum_{x_{i}^{\ell}}\prod_{\eff_{\alpha} \in \widetilde{\mathcal{B}}_{i}^{\ell}}\eff_{\alpha}(\mathbf{x}_{\alpha})\\
    &=
    r_{i}^{\ell}(x_{i})
\sum_{x_{i^{\ell}}}
r_{i^{\ell}}(x_{i^{\ell}})
\prod_{\eff_{\alpha}
    \in \mathcal{B}_{i}^{\ell}}
    \eff_{\alpha}(x_{i^{\ell}}, \mathbf{x}_{\alpha\setminus \{i\} \cup \{i^{\ell}\}}).
%\eff_{\mathcal{B}_{i}^{\ell}}(x_{i^{\ell}}, \mathbf{x}
%_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}).
\end{align*} 
We show that \eqref{eq:mbropt}
can be solved efficiently in Section \ref{subsec:complexity}. % as a low-rank approximation problem on $\eff_{\mathcal{B}_{i}^{\ell}}$. 
After all mini-buckets are processed, 
factors can be summed over 
the variables $x_{i^{1}}, \cdots, x_{i^{m_{i}-1}}$ and $x_{i}$ 
separately, i.e., 
introduce new factors as follows:
\begin{align}
    \eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}
    (\mathbf{x}_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}) 
    &=\sum_{x_{i^{\ell}}} 
    \prod_{\eff_{\alpha}\in 
    \widetilde{\mathcal{B}}_{i}^{\ell}\setminus \{r_{i}^{\ell}\}}
    \eff_{\alpha}(\mathbf{x}_{\alpha}), 
    \label{eq:mbr1}
    \\
    &= 
    \sum_{x_{i^{\ell}}}
    r^{\ell}_{i}(x_{i^{\ell}})
    \prod_{\eff_{\alpha}
    \in \mathcal{B}_{i}^{\ell}}
    \eff_{\alpha}(x_{i^{\ell}}, \mathbf{x}_{\alpha\setminus \{i\} \cup \{i^{\ell}\}}), \notag
\end{align} 
for $\ell = 1,\cdots, m_{i}-1$ 
and 
\begin{equation}\label{eq:mbr2}
\eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}
    (\mathbf{x}_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}) 
    = 
    \sum_{x_{i}}
    \prod_{\ell=1}^{m_{i}-1}r^{\ell}_{i}(x_{i^{\ell}})
    \prod_{\eff_{\alpha}
    \in \mathcal{B}_{i}^{m_{i}}}
    \eff_{\alpha}(\mathbf{x}_{\alpha}).
\end{equation}
Resulting factors are then added to 
its corresponding mini-bucket and 
repeat until all buckets are processed, like BE and MBE. 
Here, one can check that 
\begin{align*}
\prod_{\ell=1}^{m_{i}}
\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}} 
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}\setminus \{i\} })
&= 
\sum_{x_{i}}\eff_{\mathcal{B}_{i}^{m_{i}}}(\mathbf{x}_{\mathcal{B}_{i}^{m_{i}}})
\prod_{\ell=1}^{m_{i}-1}\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}),\\
&\approx
\sum_{x_{i}}
\prod_{\ell=1}^{m_{i}}\eff_{\mathcal{B}_{i}^{\ell}}(\mathbf{x}_{\mathcal{B}_{i}^{\ell}})
,
\end{align*} 
from \eqref{eq:mbropt} and MBR indeed approximates BE. 
The formal description of MBR is given in Algorithm \ref{alg:mbr}. 
%*Add a figure to illustrate?* %for a summary of the scheme. 


\input{alg1.tex}

\subsection{Complexity}
\label{subsec:complexity}
%We conclude this subsection with 
%remarks on the optimization for 
%renormalization of mini-buckets, i.e., \eqref{eq:mbropt}. 
The optimization %Each approximation 
\eqref{eq:mbropt} is related to % be interpreted as a
the rank-$1$ approximation on $\eff_{\mathcal{B}_{i}^{\ell}}$, 
which can be solved efficiently via (truncated) singular value decomposition (SVD). 
Specifically, let $\mathbf{M}$ be a $d \times d^{|\mathcal{V}(\mathcal{B}_{i}^{\ell})|-1}$ matrix representing
$\eff_{\mathcal{B}_{i}^{\ell}}$ 
as follows:
\begin{equation}\label{eq:svd}
    \mathbf{M}
    \left(
    x_{i},
    \sum_{j\in\mathcal{V}(\mathcal{B}_{i}^{\ell}), j \neq i}
    x_{j}
    \prod_{k \in \mathcal{V}(\mathcal{B}_{i}^{\ell}), k>j}d
    \right)
    =
    \eff_{\mathcal{B}_{i}^{\ell}}(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}).
\end{equation}
Then rank-1 truncated SVD for $\mathbf{M}$
solves the following optimization: %via optimization over projective truncation as follows:
%\begin{align*}
$$\min_{\mathbf{r}_{1}, \mathbf{r}_{2}}
\lVert
\mathbf{M} -
\mathbf{r}_{1}\mathbf{r}_{2}^{\top}
\mathbf{M}
\rVert_{F},$$
%\end{align*}
where optimization is over $d$-dimensional vectors $\mathbf{r}_{1}, \mathbf{r}_{2}$ and 
$\lVert\cdot\rVert_{F}$
denotes the Frobenious
norm. % of given matrix.
Namely, the solution $\mathbf{r}_{1}=\mathbf{r}_{2}$
becomes
the most significant (left) singular vector of $\mathbf{M}$, 
associated with the largest singular value.\footnote{
$\mathbf{r}_{1}=\mathbf{r}_{2}$ holds without forcing it.
} 
Especially, 
since $\mathbf{M}$ is a non-negative matrix, 
its most significant singular vector is 
always non-negative due to
the Perron-Frobenius
theorem \cite{perron1907theorie}. 
By letting $r_{i^{\ell}}(x) = \mathbf{r}_{1}(x)$ and $r_{i}^{\ell}(x) = \mathbf{r}_{2}(x)$, 
one can check that this 
optimization is 
equivalent to \eqref{eq:mbropt}, where
in fact, $r_{i^{\ell}}(x) =r_{i}^{\ell}(x)$, i.e., they share the same values.
Due to the above observations,
%As a result,  
the complexity of \eqref{eq:mbropt} is 
%solved 
%in 
$N_{\text{SVD}}(\mathbf{M})$ that denotes
the complexity of SVD for matrix $\mathbf{M}$.
%complexity %using SVD 
Therefore, the overall complexity
becomes 
$$O\left(N_{SVD}(\mathbf{M}) \cdot T\right)=
O\left(N_{\text{SVD}}(\mathbf{M})\cdot
|\mathcal{E}|\cdot\max_{\alpha \in \mathcal{E}}|\alpha|\right),$$
where
%$T:=\sum_{i\in\mathcal{V}} (m_{i}-1)$ denotes
%the number of renormalized mini-buckets 
%and
$N_{\text{SVD}}(\mathbf{M}) = O(d^{ibound+2})$ in general, but typically
much faster in the existing SVD solver. 
\iffalse
We also emphasize that 
$T$ increases as $ibound$ decreases,
and thus 
%the complexity of the algorithms 
%is more closely related to 
%the number of mini-buckets $T$  
%that are renormalized,
%i.e., 
smaller $ibound$
often lead to longer running time, as later 
discussed in Section \ref{sec:experiment}.
\fi
%the experiments.
%Hence, the complexity of MBR is exactly equal to that of MBE when $d=O(1)$, and
%we remark that any GM can be expressed as an equivalent GM with $d=2$, i.e., binary GMs of higher orders.

==> _GM Renormalization (new) (2)/main_result2.tex <==
\section{Global-Bucket Renormalization}\label{sec:global-bucket}
In the previous section, 
%we proposed the MBR scheme 
MBR  
only considers the local neighborhood
for 
renormalizing mini-buckets 
to approximate a single  marginalization 
process of BE. 
%and one might improve it
%by considering
%may not 
%necessarily 
%lead to good 
%approximation 
%of partition function, 
%due to 
%influence from other, more global
%factors %ignored  
%during 
%in the 
%renormalization process. 
%
Here we extend the approach and propose 
%Inspired by this,
%we propose an 
%improved MBR scheme, 
%namely the 
global-bucket 
renormalization (GBR), which incorporates a global perspective. %, in this section. 
The new scheme re-updates the choice of
compensating local factors 
obtained in MBR 
by considering factors 
that were 
ignored during the original process. 
In particular, GBR directly 
minimizes 
the error in the 
partition function 
from each renormalization, 
aiming for improved accuracy compared to MBR. 
%and promises to improve
%the accuracy of MBR. 
\subsection{Intuition and Key-Optimization}
\begin{figure*}[ht!]
\vspace{-0.05in}
\centering 
\begin{subfigure}[b]{0.99\linewidth}
    \centering
    \includegraphics[width=0.99\textwidth]{fig/gm_renormalization.png}
    \end{subfigure}
    \caption{Example of GM renormalization on complete graph with 
    size $|\mathcal{V}|=6$ corresponding to execution of MBR with  elimination order $o=1,\cdots,6$ and $ibound=2$. 
    Here, pairwise factors between variables are assumed 
    to exist inside edges.
    Partition function of final GM is 
    able to be computed from BE with induced width $2$ and elimination order $\widetilde{o}=[1^{a},1^{b},1,2^{a},2,3^{a},3,4,5,6]$.}
    \label{fig:gm_renormalization}
    \vspace{-0.1in}
\end{figure*}

{\bf Renormalized GMs in MBR.} 
For providing the underlying design principles of GBR,
%complete description and intof GBR, 
we first track 
an intermediate estimation 
of the partition function made during MBR by characterizing the corresponding sequence of 
renormalized GMs. 
Specifically, 
we aim for constructing a sequence of $T+1$ 
GMs 
$\mathcal{M}^{(1)},\cdots,\mathcal{M}^{(T+1)}$ with  
$T = \sum_{i=1}^{n}(m_{i}-1)$ 
by 
breaking each $i$-th iteration 
of MBR into $m_{i}-1$ steps of GM renormalizations,
$\mathcal{M}^{(1)}$ is the original GM, 
and each transition from $\mathcal{M}^{(t)}$ to $\mathcal{M}^{(t+1)}$ 
corresponds to 
renormalization of 
some mini-bucket $\mathcal{B}_{i}^{\ell}$ 
to $\widetilde{\mathcal{B}}_{i}^{\ell}$. 
Then,
the 
intermediate estimation for
the original partition function $Z$ at 
the $t$-th step 
%of renormalization 
is %as 
partition function $Z^{(t)}$ of $\mathcal{M}^{(t)}$ where 
the last one $Z^{(T+1)}$ is the output of MBR. 
\iffalse
\textcolor{red}{We point that 
similar scheme has been 
proposed in the name of 
``variable splitting'' 
in previous mini-bucket scheme, 
i.e., \citep{liu2011bounding}, 
however the corresponding 
result was not a valid GM 
and intermediate steps of 
approximations 
were not considered. 
}
\fi
%approximation given 
%by MBR by construction.


To this end, 
we introduce 
``scope'' %$\mathcal{S}_{\eff_{\alpha}}$ 
for each factor $\eff_{\alpha}$
appearing in MBR 
to indicate which parts of GM 
are renormalized at each step. % of MBR.
In particular, the scope $\mathcal{S}_{\eff_{\alpha}} 
= (\mathcal{G}_{\eff_{\alpha}}, \mathcal{F}_{\eff_{\alpha}})$ consists of a graph $\mathcal{G}_{\eff_{\alpha}} 
= (\mathcal{V}_{\eff_{\alpha}}, 
\mathcal{E}_{\eff_{\alpha}})$ 
and set of factors $\mathcal{F}_{\eff_{\alpha}}$
that are associated to $\eff_{\alpha}$ as follows: 
\begin{equation*}
\eff_{\alpha}(\mathbf{x}_{\alpha}) 
= 
\sum_{\mathbf{x}_{\mathcal{V}_{\eff_{\alpha}}\setminus\alpha}}
\prod_{\eff_{\beta}\in\mathcal{F}_{\eff_{\alpha}}}
\eff_{\beta}(\mathbf{x}_{\beta}).  
\end{equation*}
Initially, scopes associated with initial factors  
are defined by themselves, 
i.e., 
\begin{equation}\label{eq:initscope}
\mathcal{S}_{\eff_{\alpha}} \leftarrow ((\alpha,\{\alpha\}), 
\{\eff_{\alpha}\}),
\end{equation}
for each factor 
$\eff_{\alpha}$ of $\mathcal{M}^{(1)}$, 
and others of $\mathcal{M}^{(t)}= ((\mathcal V^{(t)}, \mathcal E^{(t)}), \mathcal F^{(t)})$ with $t\geq 2$ are to be defined 
iteratively under the MBR process, as we describe in what follows.



%Now we describe the 
%renormalization process explicitly 
%following the MBR process. 
Consider the $t$-th iteration of MBR, 
where mini-bucket $\mathcal{B}_{i}^{\ell}$ 
is being renormalized into 
$\widetilde{\mathcal{B}}_{i}^{\ell}$. 
Then scope $\mathcal{S}_{\eff}$ for all 
$\eff \in \mathcal{B}_{i}^{\ell}$ 
goes through renormalization by 
replacing every $i$ in the scope by $i^{\ell}$ 
as follows:
\begin{equation}\label{eq:factorrenorm}
    \widetilde{S}_{\eff}
    \leftarrow
    (\mathcal{V}_{\eff}\setminus \{i\} \cup \{i^{\ell}\}, 
    \{\bar{\alpha}| \alpha \in \mathcal{E}_{\eff}\}, 
    \{\eff_{\bar{\alpha}}|\eff_{\alpha} \in \mathcal{F}_{\eff}\}),
\end{equation}
where 
$\bar{\alpha}=\begin{cases}\alpha\setminus \{i\} \cup \{i^{\ell}\}&\mbox{ 
if}~i\in\alpha\\\qquad \alpha&\mbox{otherwise}\end{cases}$.
Then, the respective GM is 
renormalized accordingly for the change of scopes, 
in addition to compensating factors $r_{i}^{\ell}, r_{i^{\ell}}$: % as follows: 
\begin{align}
\mathcal{V}^{(t+1)} &\leftarrow \mathcal{V}^{(t)}\cup \{i^{\ell}\},\notag\\
\mathcal{E}^{(t+1)} &\leftarrow \mathcal{E}^{(t)} 
\setminus\mathcal{E}_{\mathcal{B}_{i}^{\ell}}
\cup \widetilde{\mathcal{E}}_{\mathcal{B}_{i}^{\ell}}
\cup \{\{i\}, \{i^{\ell}\}\} 
,\label{eq:gmrenorm}\\
\mathcal{F}^{(t+1)} &\leftarrow \mathcal{F}^{(t)} 
\setminus\mathcal{F}_{\mathcal{B}_{i}^{\ell}}
\cup \widetilde{\mathcal{F}}_{\mathcal{B}_{i}^{\ell}}
\cup \{r_{i}^{\ell}, r_{i^{\ell}}\}, \notag
\end{align}
where 
$\mathcal{E}_{\mathcal{B}_{i}^{\ell}} = \cup_{\eff \in \mathcal{B}_{i}^{\ell}} \mathcal{E}_{\eff}, 
$ and other union of scope components 
$\widetilde{\mathcal{E}}_{\mathcal{B}_{i}^{\ell}}, 
\mathcal{V}_{\mathcal{B}_{i}^{\ell}}, 
\widetilde{\mathcal{V}}_{\mathcal{B}_{i}^{\ell}}, 
\mathcal{F}_{\mathcal{B}_{i}^{\ell}},
\widetilde{\mathcal{F}}_{\mathcal{B}_{i}^{\ell}}$ are 
defined similarly.
Finally, 
scope 
$\mathcal{S}_{\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}}$ 
for newly generated factors 
$\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}$
%, i.e., \eqref{eq:mbr1}, 
is
\begin{equation}\label{eq:factorscope1}
\mathcal{S}_{\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}}
\leftarrow
((
\widetilde{\mathcal{V}}_{\mathcal{B}_{i}^{\ell}},
\widetilde{\mathcal{E}}_{\mathcal{B}_{i}^{\ell}}
\cup \{\{i^{\ell}\}\}
),
\widetilde{\mathcal{F}}_{\mathcal{B}_{i}^{\ell}}
\cup \{r_{i^{\ell}}\}
).
\end{equation}
Furthermore, if $\ell = m_{i}-1$, we have
%we additionally assign 
\begin{equation}\label{eq:factorscope2}
\mathcal{S}_{\eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}}
\leftarrow (
(
\mathcal{V}_{\mathcal{B}_{i}^{m_{i}}}, 
\mathcal{E}_{\mathcal{B}_{i}^{m_{i}}}
\cup \{\{i\}\}
), 
\mathcal{F}_{\mathcal{B}_{i}^{m_{i}}}
\cup \{r_{i}^{\ell}\}_{\ell=1}^{m_{i}-1}
). 
\end{equation} 
This is repeated until 
the MBR process terminates, as formally described in
Algorithm \ref{alg:mbr_renormalization}. 
\iffalse
Note that every component in  
$\mathcal{S}_{\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}}$ 
is a subset of $\mathcal{M}^{(t+1)}$, e.g., 
$\mathcal{V}_{\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}} 
\subset \mathcal{V}^{(t+1)}$, 
and the renormalizations 
are well-defined.
\fi
By construction, 
the output of MBR is equal to
the partition function of the last GM 
$\mathcal{M}^{(T+1)}$,
%with its partition functon being
%equal to approximation given by MBR, 
which is computable via BE 
with induced width smaller than $ibound + 1$ 
given elimination order 
\begin{equation}
\label{eq:elimination-order}
\widetilde{o} = 
[1^{1},\cdots,1^{m_{1}-1}, 1, \cdots, n^{1},\cdots, n^{m_{n}-1}, n].
\end{equation}
\iffalse
Repeating this process leads to a 
sequence of 
$T$ renormalized GMs 
$\mathcal{M}^{(1)},\cdots,\mathcal{M}^{(t)}$
with $T = \sum_{i=1}^{n}(m_{i}-1)$, 
where each step consists of 
replicating 
each variable $i$ 
for $m_{i}-1$ times 
and adding compensating factors 
$r_{i}^{\ell}, r_{i^{\ell}}$. 
Also, partition function $Z^{(T)}$ 
of 
the final GM 
$\mathcal{M}^{(t)}$ equals the approximation given 
by MBR, 
and 
is computable via BE 
with induced width smaller than $ibound + 1$ 
given elimination order 
$\widetilde{o} = [1^{1},\cdots,1^{m_{1}},\cdots, n^{1},\cdots, n^{m_{n}}]$ by construction. 
\fi
%Summary of this process is 
%provided in Algorithm \ref{alg:mbr_renormalization}. 
%\textcolor{red}
See Algorithm \ref{alg:mbr_renormalization} for the formal description of this process,
and Figure \ref{fig:gm_renormalization} for an example.

{\bf Optimizing intermediate approximations.}
Finally, we provide 
an explicit optimization formulation
for minimizing the 
change of 
intermediate 
partition functions 
in terms of induced factors.
%from 
%the whole graph. 
Specifically, 
for each $t$-th renormalization, i.e., 
from $\mathcal{M}^{(t)}$ 
to $\mathcal{M}^{(t+1)}$, 
we consider change of the following 
factor 
$\eff_{i}$ 
induced from global-bucket 
$%\mathcal{F}^{(t)} = 
\mathcal{F}^{(t)}$ 
%to variable $x_{i}$, 
%split into $x_{i}^{1},x_{i}^{2}$ 
%as follows:
to variable $x_{i}$ in a 
``skewed'' manner as follows: 
\iffalse
{\color{red} ... $y$-variables appear first time here, what are these? Some explanations on relations between $y$ and $x$ should be added ... my understanding (MC) is that we formally split the variable $x_i$ into two, one entering the first line of the following formula and the other the second line, right?}
\fi
\begin{align*}
    \eff_{i}(x_{i}^{(1)}, x_{i}^{(2)}) 
    :=&  \sum_{\mathbf{x}_{\mathcal{V}^{(t)}\setminus \{i\}}}
    \prod_{\eff_{\alpha}\in\mathcal{F}_{\mathcal{B}_{i}^{\ell}}}
    \eff_{\alpha}(x_{i}^{(1)}, \mathbf{x}_{\alpha\setminus \{i\}})\\
    &\cdot\prod_{\eff_{\alpha} \in \mathcal{F}^{(t)} \setminus \mathcal{F}_{\mathcal{B}_{i}^{\ell}}}
    \eff_{\alpha}(x_{i}^{(2)}, \mathbf{x}_{\alpha\setminus\{i\}}), 
\end{align*} 
where $x_{i}^{(1)},x_{i}^{(2)}$ are the 
newly introduced ``split variables'' that 
are associated with the same vertex $i$, but 
allowed to have different values 
for our purpose.
Next, the bucket $\mathcal{F}^{(t)}$ 
is renormalized into 
$\mathcal{F}^{(t+1)}$, 
leading to the induced factor of 
$\widetilde{\eff}_{i}$ 
defined as follows:
\begin{align*}
\widetilde{\eff}_{i}(x_{i}^{(1)}, x_{i}^{(2)}) 
:=& \sum_{\mathbf{x}_{\mathcal{V}^{(t+1)}\setminus \{i\}}}
    \prod_{\eff_{\alpha}\in\widetilde{\mathcal{F}}_{\mathcal{B}_{i}^{\ell}}\cup\{r_{i}^{\ell}, r_{i^{\ell}}\}}
    \eff_{\alpha}(x_{i}^{(1)}, \mathbf{x}_{\alpha\setminus \{i\}})
    \notag\\
    &\cdot \prod_{\eff_{\alpha} \in \mathcal{F}^{(t+1)} 
    \setminus \widetilde{\mathcal{F}}_{\mathcal{B}_{i}^{\ell}}\setminus \{r_{i}^{\ell}, r_{i^{\ell}}\}}
    \eff_{\alpha}(x_{i}^{(2)}, 
    \mathbf{x}_{\alpha\backslash \{i\}})\notag\\
    =&
    r_{i}^{\ell}(x_{i}^{(1)})
    \sum_{x_{i^{\ell}}}
    r_{i^{\ell}}(x_{i^{\ell}})
    \eff_{i}(x_{i^{\ell}}, x_{i}^{(2)}).
\end{align*}
Then change in $\eff_{i}$ 
is directly related with 
change in partition function since
$Z^{(t-1)}$ and $Z^{(t)}$ can 
be described as follows:
\begin{equation*}
    Z^{(t-1)} = \sum_{x_{i}}\eff_{i}(x_{i}, x_{i}), \quad
    Z^{(t)} = \sum_{x_{i}}\widetilde{\eff}_{i}(x_{i},x_{i}).
\end{equation*}
Consequently, 
GBR chooses to 
minimize the change in $\eff_{i}$ 
by re-updating 
$r_{i}^{\ell}, r_{i^{\ell}}$, i.e., 
it solves
\begin{equation}\label{eq:lbropt}
\min_{r_{i}^{\ell},r_{i^{\ell}}}
\sum_{x_{i}^{(1)},x_{i}^{(2)}} 
\bigg(
\eff_{i}(x_{i}^{(1)},x_{i}^{(2)}) 
- 
\widetilde{\eff}_{i}(x_{i}^{(1)},x_{i}^{(2)})
\bigg)^{2}.
\end{equation}
%However, we remark that 
%\eqref{eq:lbropt} 
%is intractable 
%since its objective requires 
%exponential number of 
%summation over configurations 
%$\mathbf{x}_{\mathcal{V}^{(t)}\setminus \{i\}}$.
However, we remark that \eqref{eq:lbropt} 
is intractable since 
its objective is ``global'', 
and requires summation over 
all variables except one, i.e.,  
$\mathbf{x}_{\mathcal{V}^{(t)}\setminus \{i\}}$, 
and this is the key difference from \eqref{eq:mbropt} 
which seeks to minimize 
the error described by the local mini-bucket.
GBR avoids this issue by 
substituting $\eff_{i}$ by its 
tractable approximation $\mathnormal{g}_{i}$, 
which is to be described 
in the following section.
\iffalse
{\color{red} ... I would clarify say that intractability is related to summations over all other variables than the one to be eliminated ... which complexity is equivalent to complexity of the original partition function. Even more generally,  I would probably describe here a principal difference of the global approach and local approach ... in the former (discussed here) we are seeking to minimize error in the global object, while in the latter (previous section) error-minimization was limited to the bucket only ... agree? }
\fi
\input{alg2.tex}

\subsection{Algorithm Description}
In this section, we provide a formal description of GBR.
%for 
%iteratively updating the 
%compensating factors. 
First, consider the 
sequence of GMs  
$\mathcal{M}^{(1)}, \cdots, \mathcal{M}^{(T+1)}$ 
from interpreting 
MBR as GM renormalizations. 
One can observe that this 
corresponds to 
$T$ choices of 
compensating 
factors made at each renormalization, 
i.e., $r^{(1)},\cdots, r^{(T)}$ 
where $r^{(t)}(x) = r_{i}^{\ell}(x) = r_{i^{\ell}}(x)$ 
for the associated 
replicate vertex $i^{\ell}$.
GBR modifies this sequence iteratively 
by replacing intermediate choice of 
compensation $r^{(t)}$ 
by another choice $s^{(t)}(x)=s_{i}^{\ell}(x)=s_{i^{\ell}}(x)$ 
in reversed order, 
%based on 
approximately 
solving \eqref{eq:lbropt} until 
all compensating factors are updated. 
%After every 
%compensating factors are updated, 
Then, GBR outputs partition function $Z^{(T+1)}$ 
for $\mathcal{M}^{(T+1)}$ as an approximation of the 
original partition function $Z$.

\iffalse
Specifically, at each $t^{\prime}$-th 
iteration of GBR, 
sequence of compensating factors 
$r^{(1)},\cdots,r^{(t)},s^{(t+1)},\cdots, s^{(T)}$ 
is updated into 
$r^{(1)},\cdots,r^{(t-1)},s^{(t)},\cdots, s^{(T)}$, 
where $t= T - t^{\prime}$ 
since updates are done backwards. 
Repeating this for every compensating factors, 
one arrives at 
modified 
sequence of 
renormalized GMs 
$\mathcal{M}^{(1,t^{\prime})}, \cdots \mathcal{M}^{(T, t^{\prime})}$ 
associated with $t^{\prime}$-th 
iteration of GBR, 
initially set with $\mathcal{M}^{(t,1)} = \mathcal{M}^{(t)}$. 
\fi
\iffalse
For each $t^{\prime}$-th iteration of GBR,
this sequence 
is modified by 
replacing 
intermediate 
choice of compensation 
factor $r^{(t)}$ by 
another $s^{(t)}$ by solving 
\eqref{eq:lbropt}
in reversed order. 
Then, one arrives at $T$ 
sequence of updates on compensating 
factors, 
where each set of updated 
compensating factors 
$r^{(1)},\cdots,r^{(T-t^{\prime})}, 
s^{(T-t^{\prime}+1)},\cdots, s^{(T)}$
corresponding to 
sequence of renormalized GMs 
$\mathcal{M}^{(1,t^{\prime})}, \cdots, \mathcal{M}^{(T,t^{\prime})}$ 
for each $t^{\prime} = 1,\cdots, T + 1$, 
where $\mathcal{M}^{(t,1)} = \mathcal{M}^{(t)}$. 
\fi 
\iffalse
After every compensating 
factors are processed, 
GBR outputs the partition function of final GM $\mathcal{M}^{(T+1,T+1)}$ 
as an approximation of the original partition function.
\fi
\iffalse
since compensating factors 
are dependent on its predecessors, 
i.e., $r^{(t_{1})}$ is dependent on $r^{(t_{2})}$ 
for $t_{1} > t_{2}$. 
As a result, 
GBR updates 
the choice of 
compensating factors at 
$t^{\prime}$-th iteration
without harming the 
approximating properties 
in the first $t-1$ GM 
renormalizations, i.e., 
$M^{(1,t^{\prime})},\cdots, M^{(t-1, t^{\prime})}$.
\fi

Now we describe the process of choosing 
new compensating factors 
$s_{i}^{\ell}, s_{i^{\ell}}$ 
at $t^{\prime}$-th iteration of GBR 
by approximately 
solving \eqref{eq:lbropt}. 
To this end, the $t^{\prime}$-th choice 
of compensating factors are 
expressed as follows:
\begin{equation}\label{eq:lbr1}
r^{(1)},\cdots, r^{(t)},s^{(t+1)},\cdots, s^{(T)},
\end{equation}
with $t = T- t^{\prime} + 1$ and
$s^{(t+1)},\cdots,s^{(T)}$ 
already chosen in the 
previous iteration of GBR. 
Next, 
consider sequence of GMs 
$\widehat{\mathcal M}^{(1)}, \cdots, \widehat{\mathcal M}^{(T+1)}$ 
that were generated similarly 
with GM renormalization corresponding to MBR, 
but with compensating factors chosen 
by \eqref{eq:lbr1}. 
Observe that the first $t$ 
renormalizations of GM 
correspond 
to those of MBR 
since the updates are done in reverse order, 
i.e., 
$\widehat{\mathcal M}^{(t^{\prime})} = \mathcal M^{(t^{\prime})}$ for $t^{\prime} < t + 1$. 
Next, 
$\eff_{i}$ in 
\eqref{eq:mbropt} 
is expressed as 
summation over 
$\mathbf{x}
_{\widehat{\mathcal{V}}^{(t+1)}\setminus \{i, i^{\ell}\}}
^{\ell}$ 
in $\widehat{\mathcal M}^{(t+1)}$, 
defined as follows: 
\begin{equation*}
\eff_{i}
(
x_{i^{\ell}}, 
x_{i}
) 
= 
\sum_{\mathbf{x}_{\widehat{\mathcal{V}}^{(t+1)}\setminus \{i, i^{\ell}\}}}
\prod_{\eff_{\alpha} \in \widehat{\mathcal{F}}^{(t+1)} \setminus \{r_{i}^{\ell} , r_{i^{\ell}}\}}
\eff_{\alpha}(\mathbf{x}_{\alpha}).
\end{equation*}
Since $\eff_{i}$ 
resembles the partition function 
in a way that it is also a summation  
over GM with small 
change in a set of factors, i.e., 
excluding local factors 
$r_{i}^{\ell}, r_{i^{\ell}}$, 
we expect 
$\eff_{i}$ to be 
approximated well by %that is
a summation $g_i$ over 
$\mathbf{x}_{\widehat{\mathcal{V}}^{(T+1)}\setminus \{i, i^{\ell}\}}$ 
in $\widehat{\mathcal M}^{(T+1)}$: % as follows: 
\begin{equation*}
g_{i}(x_{i^{\ell}}, x_{i}) 
:= 
\sum_{\mathbf{x}_{\widehat{\mathcal{V}}^{(T+1)} 
\setminus \{i,i^{\ell}\}}}
\prod_{\eff_{\alpha} \in \widehat{\mathcal{F}}^{(T+1)} 
\setminus \{r_{i}^{\ell}, r_{i^{\ell}}\}}
\eff_{\alpha}(\mathbf{x}_{\alpha}), 
\end{equation*} 
which can be computed in 
$O(|\mathcal{E}|d^{ibound+2})$ complexity 
via appying BE in $\widehat{\mathcal M}^{(T+1)}$ 
with elimination order 
$\widetilde{o}\setminus \{i,i^{\ell}\}$ as in 
\eqref{eq:elimination-order}.
Then 
the following optimization is obtained as an  
approximation of \eqref{eq:lbropt}:
\begin{equation}\label{eq:lbropt2}
    \min_{s_{i}^{\ell}, s_{i^{\ell}}} \sum_{x_{i}^{(1)},x_{i}^{(2)}}
    \bigg(
    g_{i}(x_{i}^{(1)},x_{i}^{(2)}) 
    -
    \widetilde{g}_{i}(x_{i}^{(1)},x_{i}^{(2)}) 
    \bigg)^{2},
\end{equation}
where $\widetilde{g}_{i}$ corresponds to renormalized factor $\widetilde{\eff}_{i}$: 
%defined as follows:
\begin{equation*}
\widetilde{g}_{i}(x_{i^{\ell}}, x_{i}) 
    :=  
    s_{i}^{\ell}(x_{i^{\ell}})
    \sum_{x_{i^{\ell}}}
    s_{i^{\ell}}(x_{i^{\ell}})
    g_{i}(x_{i^{\ell}}, x_{i}).
\end{equation*}
As a result, 
one can expect choosing compensating factors from  \eqref{eq:lbropt2} 
to improve over that of 
\eqref{eq:mbropt} as long as 
MBR provides reasonable 
approximation for $\eff_{i}$.
The optimization is again solvable via rank-$1$ 
truncated SVD 
%using $O(d^{3})$ time complexity 
and the overall complexity of GBR
is %requires 
\begin{equation*}
O\left(d^{ibound + 2} N_{\text{SVD}}(\mathbf{M}^{\text{global}}) \cdot|\mathcal{E}|^{2}\cdot \max_{\alpha \in \mathcal{E}}|\alpha|^{2}\right), 
\end{equation*}
where $N_{\text{SVD}}(\mathbf{M}^{\text{global}}) = O(d^{3})$ 
is the complexity for performing SVD on 
$d\times d$ matrix $\mathbf{M}^{\text{global}}$
representing function $g$ as in \eqref{eq:svd}.
%time complexity in overall. 
While the formal description of GBR is conceptually 
a bit complicated, one can implement it efficiently.
%its 
%actual implementation 
%is simple. 
Specifically, during the GBR process, 
it suffices to keep only the 
description of 
renormalized GM 
$\mathcal{M}^{(T+1)}$ 
with an ongoing set of 
compensating factors, 
e.g., \eqref{eq:lbr1}, 
in order to update compensating factors iteratively 
by \eqref{eq:lbropt2}. 
%Then, compensating factors 
%$r_{i}^{\ell}, r_{i^{\ell}}$ are 
%updated by solving \eqref{eq:lbropt2}, 
%with $g_{i}$ 
%being defined 
%by current set of compensating factors. 
The formal description of  the GBR scheme 
is provided in 
Algorithm \ref{alg:lbr}. 
\input{alg3.tex}

\iffalse
\textcolor{red}{
At high level, 
our algorithm 
aims to consider the 
effect of factors describing 
a larger region 
. 
Several approaches \cite{srg,gilt} have 
been proposed to 
}
\fi
\iffalse
\textcolor{red}{
Finally, we conclude this section with 
comparison of GBR to prior tensor 
network renormalization 
methods. 
Minimizing the 
renormalization error 
for partition function 
explicitly have been 
first considered in the so-called 
name of second-order renormalization groups \cite{xie2009second, xie2012coarse}. 
While schematically different, e.g., updates are not done in revers order, 
such works can be considered as an 
alternative modifications for the GBR. 
Further, this framework was 
later generalized into a more complex renormalization of sub-networks, i.e., bucket, 
with arbitrary size  \cite{evenbly2015tensor, hauru2018renormalization}. 
Extension of these works to Factor-graph GMs 
is of future interest. 
}
{\color{red} ... not sure if this is a good place for this discussion (possibly conclusions turned into conclusions+path forward would be a better place ... but I would certainly like to cite the "Renormalization of tensor networks using graph independent local truncations" by Hauru et al 2017, as an example from physics literature where local optimization was replaced by global ... I still believe that the scheme of the paper is different from ours ... in the physics jargon it comes (and is explained clearly in the paper) as "removing ultra-violet/small-scale details or local correlations" considering effect on a tensor (factor) which describes a region which is larger then the current bucket. I think the scheme of the physics paper can be viewed as an alternative modification of what is described in section 4.1. Specifically, $f_i$ and $\tilde{f}_i$ in Eq.(7), which is not tractable, would be replaced by comparison of tensors describing not the whole graph/problem, but only a region. In any case this story is not for the paper. What I suggest is just to have a remark that other approximations of $f$ from (7) are possible, and some of them are discussed in the aforementioned physics papers. May be also adding that further exploration of other options is left for future research.  }
\fi
\iffalse
\textcolor{blue}{Sungsoo: I tried to answer the remark in 
end of section 4.1... Please let me know if this is not a good place or there is more to be added.}
\fi


\iffalse
Several previous 
works in tensor network renormalization 
\cite{xie2009second, xie2012coarse, hauru2018renormalization} have 
considered objectives 
similar to \eqref{eq:lbropt}, 
minimizing the renormalization error 
defined on network (i.e., bucket) 
describing a 
larger region. 
While schematically different, 
such works 
can be considered as an 
alternative modifications 
for the GBR.
\fi

\iffalse
Then for each 
In order to indicate which parts of $\mathcal{M}^{(t)}$ 
is transformed along with the mini-bucket, 
we keep track of ``scope'' 
$\mathcal{S}_{\eff_{\alpha}} 
= (G_{\eff_{\alpha}}, \mathcal{F}_{\eff_{\alpha}})
$ 
with subgraph $G_{\eff_{\alpha}} 
= (\mathcal{V}_{\eff_{\alpha}}, 
\mathcal{E}_{\eff_{\alpha}})$ 
for each factor $\eff_{\alpha}\in\mathcal{B}_{i}^{\ell}$ 
that makes up the corresponding factor, 
i.e., 
\begin{equation*}
\eff_{\alpha}(\mathbf{x}_{\alpha}) 
= 
\sum_{\mathbf{x}_{\mathcal{V}_{\eff_{\alpha}}-\alpha}}
\prod_{\eff_{\beta}\in\mathcal{F}_{\eff_{\alpha}}}
\eff_{\beta}(\mathbf{x}_{\beta}),
\end{equation*} 
where 
$\mathcal{V}_{\eff_{\alpha}} \subset \mathcal{V}^{(t)}, \mathcal{E}_{\eff_{\alpha}} \subset \mathcal{E}^{(t)},
\mathcal{F}_{\eff_{\alpha}} \subset \mathcal{F}^{(t)}$ 
indicate set of vertices, hyper-edges, factors in $\mathcal{M}^{(t)}$ 
associated with $\eff_{\alpha}$ respectively. 
\fi
\iffalse
Next, we additionally 
associate scope for mini-bucket $\mathcal{B}_{i}^{\ell}$, 
i.e., $\mathcal{S}_{\mathcal{B}_{i}^{\ell}}$,
which indicates union 
of scopes for factors in the set, 
i.e., 
\begin{equation*}
\mathcal{S}_{\mathcal{B}_{i}^{\ell}} 
\leftarrow 
(
(
\cup_{\eff\in\mathcal{B}_{i}^{\ell}} 
\mathcal{V}_{\eff},
\cup_{\eff\in\mathcal{B}_{i}^{\ell}} 
\mathcal{E}_{\eff}
)
,\cup_{\eff\in\mathcal{B}_{i}^{\ell}} 
\mathcal{F}_{\eff}
).
\end{equation*}
We remark that 
$\mathcal{V}_{\mathcal{B}_{i}^{\ell}}$ 
can be confused with $\mathcal{V}(\mathcal{B}_{i}^{\ell})$ 
due to abuse of notation. 
However, $\mathcal{V}(\mathcal{B}_{i}^{\ell})$ 
are only 
defined on variables existing in 
intermediate stage of MBR while 
$\mathcal{V}_{\mathcal{B}_{i}^{\ell}}$ 
also includes the variables 
that were eliminated in previous 
iteration of MBR. 
Especially, 
one can check that 
$\mathcal{V}(\mathcal{B}_{i}^{\ell}) \subset \mathcal{V}_{\mathcal{B}_{i}^{\ell}}$.
\fi
\iffalse
Now we follow the process of MBR 
while ignoring the elimination process, 
where we renormalize the GM 
by replacing the scope associated with 
each mini-bucket renormalization.
Specifically, the scope of factor 
in the original GM are initially 
set by itself, i.e., 
$\mathcal{S}_{\eff_{\alpha}}= ((\alpha,\{\alpha\}), 
\{\eff_{\alpha}\})$ for 
$\eff_{\alpha}\in \mathcal{F}$.
Next, for each 
mini-bucket $\mathcal{B}_{i}^{\ell}$ 
being renormalized, i.e., $\ell < m_{i}$,
the corresponding 
components of GM will be 
renormalized along with it, 
i.e., 
\fi

==> _GM Renormalization (new) (2)/main_result2_old2.tex <==
\section{Second-Order Mini-Bucket Renormalization}
In this section, 
we propose a 
second-order 
mini-bucket renormalization 
algorithm 
to improve upon bare MBR. 
While MBR choose the 
reweighting 
functions by 
minimizing 
the error from 
splitting a 
bucket into multiple  mini-buckets, 
its optimization is based on 
local neighbors of each variable 
and there may exist a better choice for approximating the partition function. 
Inspired by this, 
second-order MBR 
attempts to minimize the 
approximation error 
of partition function 
directly. 

The rest of this section 
consists of two parts. 
First, in order to obtain an explicit description of 
the partition function approximation error made by MBR, 
we interpret the algorithm  
as a sequence of GM renormalization. 
Next, we provide the 
explicit partition function approximation error and 
describe the second-order MBR 
for minimizing it.

\subsection{MBR as GM renormalizaton}
In order to provide an explicit 
description on 
partition function approximation 
error made by MBR, 
we interpret each 
elimination process of 
MBR as a series 
of ``renormalization'' operations 
on GM, where at each step, 
components of the GM is 
modified by 
splitting variables 
and adding local factors. 

To this end, we observe 
that renormalization of 
each mini-bucket 
\eqref{eq:eq1} can be 
reformulated as follows:
\begin{align*}
\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) &= 
    r_{i}^{\ell}(x_{i})
\sum_{x_{i^{\ell}}}
r_{i^{\ell}}(x_{i^{\ell}})
\prod_{\eff_{\alpha} \in \mathcal{B}_{i}^{\ell}}\eff_{\alpha}(x_{i^{\ell}}, \mathbf{x}
_{\alpha\backslash i}).
\end{align*} 
This procedure can be seen as a transformation of GM, where every 
vertex $i$ in mini-bucket  $\mathcal{B}_{i}^{\ell}$ is replaced 
by its replicate $i^{\ell}$, 
and then adding new local factors $r_{i}^{\ell}, r_{i^{\ell}}$ 
to compensate. 
We also assume 
that the corresponding 
graph is updated accordingly. 
As a result, 
elimination of variable 
$x_{i}$ can be seen as 
$m_{i}-1$ steps of variable splitting and compensating, 
followed by 
one variable elimination stage. 
Finally, we obtain a sequence of GMs 
$(G^{(0)}, \mathcal{F}^{(0)}), \cdots, (G^{(T)}, \mathcal{F}^{(T)})$ 
for $T = \sum_{i=1}^{n}m_{i}$ 
such that at $t$-th iteration 
where $t = \sum_{j=1}^{i-1}m_{i} + \ell -1$ with $1 \leq \ell < m_{i}$, 
GM defined on $(G^{(t)}, \mathcal{F}^{(t)})$ is 
transformed by 
replacing the mini-bucket $\mathcal{B}_{i}^{\ell}$ by 
a new one with replicate vertex $i^{\ell}$ and compensating local factors $r_{i}^{\ell}, r_{i^{\ell}}$.
Otherwise if 
$t = \sum_{j=1}^{i}m_{i}$, 
variable $x_{i}$ and its replicates $x_{i^{1}},\cdots, x_{i^{m_{i}-1}}$ 
are eliminated by marginalization. 
At final iteration, 
we observe that the partition function 
approximation given by MBR can be expressed as $Z^{(T)} = \prod_{\alpha\in\mathcal{F}^{(T)}}\eff_{\alpha}$. 
As a result, 
one can interpret 
the approximation 
error made by splitting 
each mini-bucket as a difference of 
partition function between subsequent GMs.


\subsection{Description of second-order renormalization}
In the Section \eqref{sec:rmbe}, 
we observed that 
first-order MBR, 
i.e., bare MBR, 
corresponds to 
replacement of 
scopes for each mini-bucket, 
with minimal change 
in corresponding variables. 
Now we describe the second-order mini-bucket renormalization, 
which 
attempts to 
choose the local factors 
by minimizing 
the change of 
partition function $Z$ 
between subsequent GMs 
most directly. 

Consider $t$-th 
iteration of the 
second-order MBR, 
corresponding to 
GM defined on 
$(G^{(t)}, \mathcal{F}^{(t)})$ 
where 
$t = \sum_{j=1}^{i-1}m_{i} + \ell$ with 
$1\leq \ell < m_{i}$. 
Then its 
partition function 
$Z^{(t)}$
can 
be expressed 
as follows:
\begin{align*}
Z^{(t)} &= 
\sum_{x_{i}} 
g(x_{i},x_{i}), \\
g(x_{i},y_{i}) &= 
\sum_{\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}}
\eff_{\mathcal{B}_{i}^{\ell}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) \bar{\eff}_{\mathcal{B}_{i}^{\ell}}
(y_{i}, 
\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}).
\end{align*} 
Here, $\eff_{\mathcal{B}_{i}^{\ell}}$ is as defined in \eqref{eq:factorrenorm} 
and $\bar{\eff}_{\mathcal{B}_{i}^{\ell}}$ is 
marginalization over 
components in 
$(G^{(t)}, \mathcal{F}^{(t)})$ 
that is complementary  $\eff_{\mathcal{B}_{i}^{\ell}}$, 
defined as follows:
\begin{equation*}
\bar{\eff}_{\mathcal{B}_{i}^{\ell}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) 
= 
\sum_{\mathbf{x}_{\mathcal{V}^{(t)}\backslash 
\mathcal{B}_{i}^{\ell}}}
\prod_{\alpha \in \mathcal{E}^{(t)} - \mathcal{B}_{i}^{\ell}}
\eff_{\alpha}(\mathbf{x}_{\alpha}).
\end{equation*}

Moreover, 
the partition function of 
$(t+1)$-th GM will 
be expressed as follows: 
\begin{align*}
Z^{(t+1)} 
&= 
\sum_{x_{i}}
\widetilde{g}(x_{i},x_{i}),\\
\widetilde{g}(x_{i},y_{i}) &= 
\sum_{\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}}
\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) 
\bar{\eff}_{\mathcal{B}_{i}^{\ell}}
(y_{i}, 
\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}), 
\end{align*} 
where $\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}$ is as defined in \eqref{eq:factorrenorm}. 
This implies that 
in order to reduce 
the error in partition function 
from transformation of GMs more directly, 
one needs to minimize the change in 
function $g$ instead of \eqref{eq:mbropt}. 
That is, 
optimal choice 
of update for 
$r_{i}^{\ell}, r_{i^{\ell}}$ 
should be chosen as 
solution of the following problem: 
\begin{equation*}
\min_{r_{i}^{\ell}, r_{i^{\ell}}} 
\sum_{x, y} 
\bigg(
g(x_{i},y_{i}) 
- 
\widetilde{g}(x_{i},y_{i})
\bigg)^{2}. 
\end{equation*} 
This optimization can be 
seen as improving \eqref{eq:mbr2} 
by using information over the global structure of GM. 
However, computational 
complexity arise since $\bar{\eff}_{\mathcal{B}_{i}^{\ell}}$ 
requires 
summation over 
exponential number of 
configurations in 
$t$-th GM 
that are not yet 
renormalized. 

To resolve this issue, 
we propose to solve 
an approximated optimization 
where $g$ and $\widetilde{g}$ are  
approximated using 
first-order MBR. 
To this end, 
we observe that 
one can 
assign an auxiliary GM 
to functions 
$g$ 
so that it is defined as its marginals as 
follows:

Then the rest of algorithm can be defined as follows:
For each pair of variable $i$ in elimination order and mini-bucket $\mathcal{B}_{i}^{\ell}$, 
one estimates the description of corresponding 
$h$ and $\widetilde{h}$ by running 
MBR on the auxiliary GM. 
Then, the GM is updated with 
local factors chosen from \eqref{eq:secondmbropt}. 
This scheme is summarized in Algorithm \ref{alg:xx}. 

==> _GM Renormalization (new) (2)/preliminary.tex <==

\section{Preliminaries}
{\bf Graphical model.}
Consider a hyper-graph
$\mathcal{G} = (\mathcal{V}, \mathcal{E})$ with
vertices $\mathcal{V} = \{1,\cdots,n\}$ and
hyper-edges $\mathcal{E} \subset 2^{\mathcal V}$. A graphical 
model (GM) $\mathcal{M}= (\mathcal G, \mathcal{F})$ associates a 
collection of  $n$ discrete random variables
$\mathbf{x}=[x_{i}: i \in \mathcal{V}]\in\mathcal{X}_{\mathcal{V}}=\prod_{i\in\mathcal{V}}\mathcal{X}_{i}$
with the following joint probability distribution:
\begin{equation*}
\text{Pr}(\mathbf{x}) =
\frac{1}{Z}\prod_{\alpha\in\mathcal{E}}
\eff_{\alpha}(\mathbf{x}_{\alpha}),
\quad\quad
Z = \sum_{\mathbf{x}}
\prod_{\alpha\in\mathcal{E}}
\eff_{\alpha}(\mathbf{x}_{\alpha}),
\label{Forney}
\end{equation*}
where
$\mathcal{X}_{i}=\{1,2,\cdots d_i\}$,
$\mathbf{x}_{\alpha} = [x_{i}:i\in \mathbf{\alpha}]$,
$\mathcal{F} = \{\eff_{\alpha}\}_{\alpha \in \mathcal{E}}$
is a set of non-negative functions called {\it factors}, %functions
and $Z$ is the normalizing constant called the {\it partition function}
that is computationally intractable.
%The partition function is essential for many inference tasks of GM, e.g., sampling and
%marginalization, but it is in general computationally
%intractable, i.e., \#P-hard, even to approximate \cite{jerrum1993polynomial}.

\begin{algorithm}[ht!]
\caption{Bucket Elimination (BE)}
\label{alg:bucket}
\begin{algorithmic}[1]
\STATE {\bf Input:} GM $\mathcal{M}^{\dagger}=(\mathcal{G}^{\dagger}, \mathcal{F}^{\dagger})$
and elimination order $o$.
\vspace{0.05in}
  \hrule
    \vspace{0.05in}
\STATE $\mathcal{F} \leftarrow \mathcal{F}^{\dagger}$
\FOR{$i$ in $o$}
\STATE $\mathcal{B}_{i} 
\leftarrow \{\eff_{\alpha}|\eff_{\alpha}\in \mathcal{F}, i \in \alpha \}$
\STATE Generate new factor $\eff_{\mathcal{B}_{i}\setminus \{i\}}$ by \eqref{eq:be}.
%\begin{equation*}
%\eff_{\mathcal{B}_{i}\setminus \{i\}}
%(\mathbf{x}_{\mathcal{B}_{i}\setminus \{i\}}) = 
%    \sum_{x_{i}}\prod_{\eff_{\alpha}\in \mathcal{B}_{i}}\eff_{\alpha}(\mathbf{x}_{\alpha}), ~\forall~ %\mathbf{x}_{\mathcal{B}_{i}\setminus \{i\}}.
%    \end{equation*}
\STATE $\mathcal{F} \leftarrow \mathcal{F} \cup \{\eff_{\mathcal{B}_{i}\setminus \{i\}}\} \setminus \mathcal{B}_{i}$
\ENDFOR
\vspace{0.05in}
  \hrule
  \vspace{0.05in}
\STATE {\bf Output:} $Z = \prod_{\eff_{\alpha}\in \mathcal{F}}\eff_{\alpha}$
\end{algorithmic}
\end{algorithm}

{\bf Mini-bucket elimination.}
{\it Bucket (or variable) elimination} (BE,  \citealp{dechter1999bucket, koller2009probabilistic}) is
a procedure for computing the partition function exactly 
based on sequential elimination of variables. 
%\textcolor{red}{In general, number of variables decreases but complexity of the factors increases, thus making the exact elimination intractable.}
Without loss of generality, 
we assume through out the paper that the elimination order is fixed $o = [1,\cdots,n]$. 
BE groups factors by placing each 
factor $\eff_{\alpha}$ in the 
``bucket'' $\mathcal{B}_{i}\subset \mathcal F$ of its 
earliest argument 
$i\in \alpha$ 
appearing in the elimination order $o$.
Next, BE eliminates the variable by introducing a new factor
marginalizing the product of factors in it, 
i.e., 
\begin{equation}\label{eq:be}
\eff_{\mathcal{B}_{i}\setminus \{i\}}
(\mathbf{x}_{\mathcal{B}_{i}\setminus \{i\}})
= \sum_{x_{i}}
\prod_{\eff_{\alpha}\in \mathcal{B}_{i}}
\eff_{\alpha}(\mathbf{x}_{\alpha}).
\end{equation}
Here,
$\mathbf{x}_{\mathcal{B}_{i}\setminus \{i\}}$
abbreviates %for
$\mathbf{x}_{\mathcal{V}(\mathcal{B}_{i})\setminus \{i\}}$,
where $\mathcal{V}(\mathcal{B}_{i})$
indicates the set of variables associated with the
bucket $\mathcal{B}_{i}$.
The subscript in
$\eff_{\mathcal{B}_{i}\setminus \{i\}}$
represents a similar abbreviation.
Finally, the new %ly generated 
function $\eff_{\mathcal{B}_{i}\setminus \{i\}}$ 
is added to another bucket 
corresponding to its earliest argument in the 
elimination order. 
Formal description of BE is given
in Algorithm \ref{alg:bucket}.


One can easily check that BE 
applies a distributive property for computing $Z$ exactly:
groups of factors corresponding to buckets
are summed out sequentially,
and then the newly generated factor
(without the eliminated variable) is
added to another bucket. 
The computational cost of BE is
exponential with respect 
to the number of
uneliminated variables 
in the bucket, i.e., its complexity is 
%\begin{equation*}
$O\left(d^{\max_{i}|\mathcal{V}(\mathcal{B}_{i})|}|\mathcal{V}|\right).$
%\end{equation*}
Here, 
$\max_{i\in\mathcal{V}}|\mathcal{V}(\mathcal{B}_{i})|$ is 
called the
{\it induced width} 
of $\mathcal{G}$
given the elimination order $o$, and the minimum possible
induced width across all possible $o$ 
is called the {\it tree-width}. 
Furthermore, 
we remark that 
summation of GM over variables defined on the subset of vertices $\alpha$, 
i.e., $\sum_{\mathbf{x}_{\alpha}}\prod_{\beta\in\mathcal{E}}\eff_{\beta}$, 
can also be computed via BE 
in 
$
O(d^{\max_{i}|\mathcal{V}(\mathcal{B}_{i})| + |\mathcal{V}\setminus\alpha|}|\mathcal{V}|)
$ time by summing out variables in 
elimination order 
$o_{\alpha}$ on $\alpha$.




{\it Mini-bucket elimination} (MBE,  \citealp{dechter2003mini})
achieves lower complexity by
approximating each step of BE by
splitting the computation
of each bucket into several
smaller ``mini-buckets''.
%\citep{dechter2003mini} used the upper bound
%where the summation operator is
%applied to one mini-bucket and
%maximum is applied to all others.
Formally, for each variable $i$ in the 
elimination order $o$, 
the bucket $\mathcal{B}_{i}$ 
is partitioned into
$m_{i}$ mini-buckets
$\{\mathcal{B}_{i}^{\ell}\}_{\ell=1}^{m_{i}}$
such that 
$\mathcal{B}_{i} = \bigcup_{\ell=1}^{m_{i}}\mathcal{B}_{i}^{\ell}$ and $\mathcal{B}_{i}^{\ell_{1}}\cap \mathcal{B}_{i}^{\ell_{2}}=\emptyset$
for any $\ell_{1},\ell_{2}$.
Next, MBE generates new factors differently from BE as follows:
\begin{align}
     \eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}
     (\mathbf{x}_{\mathcal{B}_{i}^{\ell}\setminus \{i\}})
     =
     \max_{x_{i}}
     \prod_{\eff_{\alpha} \in \mathcal{B}^{\ell}_{i}}
     \eff_{\alpha}(\mathbf{x}_{\alpha}),\label{eq:mbemax}
\end{align}
for all $\ell = 1,\cdots, m_{i}-1$ and
\begin{align}
     \eff_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}}
     (\mathbf{x}_{\mathcal{B}_{i}^{m_{i}}\setminus \{i\}})
     =
     \sum_{x_{i}}
     \prod_{\eff_{\alpha} \in \mathcal{B}^{m_{i}}_{i}}
     \eff_{\alpha}(\mathbf{x}_{\alpha}).\label{eq:mbesum}
\end{align}
Other steps are equivalent to that of BE.
%Then, new factors are added to other 
%buckets. 
Observe that 
MBE %This is equivalent to 
replaces the exact marginalization of the bucket
in \eqref{eq:be}
by its upper bound,
i.e.,
$\sum_{x_{i}}
\prod_{\eff_{\alpha}\in\mathcal{B}_{i}}\eff_{\alpha}
\leq
\prod_{\ell=1}^{m}
\eff_{\mathcal{B}_{i}^{\ell}\setminus \{i\}}
$, 
and hence yields an
upper bound of $Z$. 
We remark that
one could instead obtain
a lower bound for $Z$
by replacing $\max$
by $\min$ in \eqref{eq:mbemax}.

Note that one has to choose mini-buckets for MBE carefully
as their sizes typically %(not always) 
determine complexity and accuracy:
smaller mini-buckets may be better for speed,
but worse in accuracy. 
Accordingly, MBE has an additional 
induced width bound parameter 
%The complexity of MBE is determined by
%a parameter
$ibound$ as the maximal size of a mini-bucket, 
i.e.,
$|\mathcal{V}(\mathcal{B}_{i}^{\ell})|\leq
ibound + 1$. 
%The parameter controls the cost-accuracy trade-off, i.e.,
The time complexity of MBE is %given as
$O\left(d^{ibound+1}|\mathcal{E}|\cdot \max_{\alpha\in\mathcal{E}} |\alpha| \right), $
since the maximum number of mini-buckets is bounded by $|\mathcal{E}|\max_{\alpha\in\mathcal{E}} |\alpha|$.
%where $\delta$ is maximum size of hyper-edge, i.e., $\max_{\alpha\in\mathcal{E}} |\alpha|$,
%since maximum number of mini-buckets 
%appearing in the algorithm 
%is bounded by $O(\delta|\mathcal{E}|)$. 


==> main_result2_old2.tex <==
\section{Second-Order Mini-Bucket Renormalization}
In this section, 
we propose a 
second-order 
mini-bucket renormalization 
algorithm 
to improve upon bare MBR. 
While MBR choose the 
reweighting 
functions by 
minimizing 
the error from 
splitting a 
bucket into multiple  mini-buckets, 
its optimization is based on 
local neighbors of each variable 
and there may exist a better choice for approximating the partition function. 
Inspired by this, 
second-order MBR 
attempts to minimize the 
approximation error 
of partition function 
directly. 

The rest of this section 
consists of two parts. 
First, in order to obtain an explicit description of 
the partition function approximation error made by MBR, 
we interpret the algorithm  
as a sequence of GM renormalization. 
Next, we provide the 
explicit partition function approximation error and 
describe the second-order MBR 
for minimizing it.

\subsection{MBR as GM renormalizaton}
In order to provide an explicit 
description on 
partition function approximation 
error made by MBR, 
we interpret each 
elimination process of 
MBR as a series 
of ``renormalization'' operations 
on GM, where at each step, 
components of the GM is 
modified by 
splitting variables 
and adding local factors. 

To this end, we observe 
that renormalization of 
each mini-bucket 
\eqref{eq:eq1} can be 
reformulated as follows:
\begin{align*}
\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) &= 
    r_{i}^{\ell}(x_{i})
\sum_{x_{i^{\ell}}}
r_{i^{\ell}}(x_{i^{\ell}})
\prod_{\eff_{\alpha} \in \mathcal{B}_{i}^{\ell}}\eff_{\alpha}(x_{i^{\ell}}, \mathbf{x}
_{\alpha\backslash i}).
\end{align*} 
This procedure can be seen as a transformation of GM, where every 
vertex $i$ in mini-bucket  $\mathcal{B}_{i}^{\ell}$ is replaced 
by its replicate $i^{\ell}$, 
and then adding new local factors $r_{i}^{\ell}, r_{i^{\ell}}$ 
to compensate. 
We also assume 
that the corresponding 
graph is updated accordingly. 
As a result, 
elimination of variable 
$x_{i}$ can be seen as 
$m_{i}-1$ steps of variable splitting and compensating, 
followed by 
one variable elimination stage. 
Finally, we obtain a sequence of GMs 
$(G^{(0)}, \mathcal{F}^{(0)}), \cdots, (G^{(T)}, \mathcal{F}^{(T)})$ 
for $T = \sum_{i=1}^{n}m_{i}$ 
such that at $t$-th iteration 
where $t = \sum_{j=1}^{i-1}m_{i} + \ell -1$ with $1 \leq \ell < m_{i}$, 
GM defined on $(G^{(t)}, \mathcal{F}^{(t)})$ is 
transformed by 
replacing the mini-bucket $\mathcal{B}_{i}^{\ell}$ by 
a new one with replicate vertex $i^{\ell}$ and compensating local factors $r_{i}^{\ell}, r_{i^{\ell}}$.
Otherwise if 
$t = \sum_{j=1}^{i}m_{i}$, 
variable $x_{i}$ and its replicates $x_{i^{1}},\cdots, x_{i^{m_{i}-1}}$ 
are eliminated by marginalization. 
At final iteration, 
we observe that the partition function 
approximation given by MBR can be expressed as $Z^{(T)} = \prod_{\alpha\in\mathcal{F}^{(T)}}\eff_{\alpha}$. 
As a result, 
one can interpret 
the approximation 
error made by splitting 
each mini-bucket as a difference of 
partition function between subsequent GMs.


\subsection{Description of second-order renormalization}
In the Section \eqref{sec:rmbe}, 
we observed that 
first-order MBR, 
i.e., bare MBR, 
corresponds to 
replacement of 
scopes for each mini-bucket, 
with minimal change 
in corresponding variables. 
Now we describe the second-order mini-bucket renormalization, 
which 
attempts to 
choose the local factors 
by minimizing 
the change of 
partition function $Z$ 
between subsequent GMs 
most directly. 

Consider $t$-th 
iteration of the 
second-order MBR, 
corresponding to 
GM defined on 
$(G^{(t)}, \mathcal{F}^{(t)})$ 
where 
$t = \sum_{j=1}^{i-1}m_{i} + \ell$ with 
$1\leq \ell < m_{i}$. 
Then its 
partition function 
$Z^{(t)}$
can 
be expressed 
as follows:
\begin{align*}
Z^{(t)} &= 
\sum_{x_{i}} 
g(x_{i},x_{i}), \\
g(x_{i},y_{i}) &= 
\sum_{\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}}
\eff_{\mathcal{B}_{i}^{\ell}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) \bar{\eff}_{\mathcal{B}_{i}^{\ell}}
(y_{i}, 
\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}).
\end{align*} 
Here, $\eff_{\mathcal{B}_{i}^{\ell}}$ is as defined in \eqref{eq:factorrenorm} 
and $\bar{\eff}_{\mathcal{B}_{i}^{\ell}}$ is 
marginalization over 
components in 
$(G^{(t)}, \mathcal{F}^{(t)})$ 
that is complementary  $\eff_{\mathcal{B}_{i}^{\ell}}$, 
defined as follows:
\begin{equation*}
\bar{\eff}_{\mathcal{B}_{i}^{\ell}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) 
= 
\sum_{\mathbf{x}_{\mathcal{V}^{(t)}\backslash 
\mathcal{B}_{i}^{\ell}}}
\prod_{\alpha \in \mathcal{E}^{(t)} - \mathcal{B}_{i}^{\ell}}
\eff_{\alpha}(\mathbf{x}_{\alpha}).
\end{equation*}

Moreover, 
the partition function of 
$(t+1)$-th GM will 
be expressed as follows: 
\begin{align*}
Z^{(t+1)} 
&= 
\sum_{x_{i}}
\widetilde{g}(x_{i},x_{i}),\\
\widetilde{g}(x_{i},y_{i}) &= 
\sum_{\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}}
\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}
(\mathbf{x}_{\mathcal{B}_{i}^{\ell}}) 
\bar{\eff}_{\mathcal{B}_{i}^{\ell}}
(y_{i}, 
\mathbf{x}_{\mathcal{B}_{i}^{\ell}\backslash i}), 
\end{align*} 
where $\widetilde{\eff}_{\mathcal{B}_{i}^{\ell}}$ is as defined in \eqref{eq:factorrenorm}. 
This implies that 
in order to reduce 
the error in partition function 
from transformation of GMs more directly, 
one needs to minimize the change in 
function $g$ instead of \eqref{eq:mbropt}. 
That is, 
optimal choice 
of update for 
$r_{i}^{\ell}, r_{i^{\ell}}$ 
should be chosen as 
solution of the following problem: 
\begin{equation*}
\min_{r_{i}^{\ell}, r_{i^{\ell}}} 
\sum_{x, y} 
\bigg(
g(x_{i},y_{i}) 
- 
\widetilde{g}(x_{i},y_{i})
\bigg)^{2}. 
\end{equation*} 
This optimization can be 
seen as improving \eqref{eq:mbr2} 
by using information over the global structure of GM. 
However, computational 
complexity arise since $\bar{\eff}_{\mathcal{B}_{i}^{\ell}}$ 
requires 
summation over 
exponential number of 
configurations in 
$t$-th GM 
that are not yet 
renormalized. 

To resolve this issue, 
we propose to solve 
an approximated optimization 
where $g$ and $\widetilde{g}$ are  
approximated using 
first-order MBR. 
To this end, 
we observe that 
one can 
assign an auxiliary GM 
to functions 
$g$ 
so that it is defined as its marginals as 
follows:

Then the rest of algorithm can be defined as follows:
For each pair of variable $i$ in elimination order and mini-bucket $\mathcal{B}_{i}^{\ell}$, 
one estimates the description of corresponding 
$h$ and $\widetilde{h}$ by running 
MBR on the auxiliary GM. 
Then, the GM is updated with 
local factors chosen from \eqref{eq:secondmbropt}. 
This scheme is summarized in Algorithm \ref{alg:xx}. 
